Gravitational bremsstrahlung in plasmas and clusters

We study the gravitational bremsstrahlung owing to collisions mediated by a $1/r$ potential. We combine classical and first order Born approximation results in order to construct an approximate gravitational `Gaunt factor' for the total emitted energy. We also obtain the cross-section with an angular momentum cut-off, and hence the cross-section for emission via close hyperbolic encounters in a gravitating cluster. These effects are the dominant source of very high frequency gravitational noise in the solar system. The total gravitational wave power of the Sun is $76\pm 20\,$MW.

==> chiCoul.tex <==
\begin{loglogaxis}[
xmin= 0.0001, xmax= 1,
ymin= 0.01, ymax= 1000,
xlabel={$v/c$},
ylabel={$\chi$},
ylabel near ticks,
]
\addplot [black]
coordinates {
( 0.0001, 0.999918094)
( 0.000108480964, 0.9999001)
( 0.000117681195, 0.999878202)
( 0.000127661695, 0.999851569)
( 0.000138488637, 0.999819198)
( 0.000150233808, 0.999779879)
( 0.000162975083, 0.999732159)
( 0.000176796941, 0.999674286)
( 0.000191791026, 0.999604162)
( 0.000208056754, 0.999519273)
( 0.000225701972, 0.999416613)
( 0.000244843675, 0.999292597)
( 0.000265608778, 0.999142954)
( 0.000288134963, 0.998962617)
( 0.000312571585, 0.998745579)
( 0.000339080668, 0.99848475)
( 0.000367837977, 0.998171777)
( 0.000399034183, 0.997796859)
( 0.000432876128, 0.997348531)
( 0.000469588196, 0.996813436)
( 0.000509413801, 0.996176076)
( 0.000552617002, 0.995418548)
( 0.00059948425, 0.99452027)
( 0.000650326293, 0.993457702)
( 0.000705480231, 0.992204074)
( 0.000765311755, 0.990729123)
( 0.000830217568, 0.988998861)
( 0.00090062802, 0.986975388)
( 0.000977009957, 0.984616764)
( 0.00105986982, 0.981876965)
( 0.001149757, 0.978705941)
( 0.00124726747, 0.975049803)
( 0.00135304777, 0.970851158)
( 0.00146779927, 0.966049615)
( 0.00159228279, 0.960582473)
( 0.00172732372, 0.954385608)
( 0.00187381742, 0.947394557)
( 0.0020327352, 0.939545797)
( 0.00220513074, 0.930778193)
( 0.00239214708, 0.921034592)
( 0.00259502421, 0.910263514)
( 0.00281510728, 0.898420891)
( 0.00305385551, 0.885471776)
( 0.00331285189, 0.87139197)
( 0.00359381366, 0.856169471)
( 0.0038986037, 0.839805675)
( 0.00422924287, 0.822316279)
( 0.00458792343, 0.803731797)
( 0.00497702356, 0.784097675)
( 0.00539912314, 0.763473976)
( 0.00585702082, 0.741934621)
( 0.00635375264, 0.719566234)
( 0.0068926121, 0.696466602)
( 0.00747717205, 0.672742839)
( 0.00811130831, 0.648509309)
( 0.00879922544, 0.623885402)
( 0.00954548457, 0.598993236)
( 0.0103550337, 0.573955393)
( 0.0112332403, 0.548892746)
( 0.0121859274, 0.523922448)
( 0.0132194115, 0.49915616)
( 0.014340545, 0.474698523)
( 0.0155567614, 0.450645932)
( 0.0168761248, 0.427085597)
( 0.0183073828, 0.404094909)
( 0.0198600253, 0.381741077)
( 0.0215443469, 0.360081031)
( 0.0233715152, 0.339161546)
( 0.0253536449, 0.319019565)
( 0.0275038784, 0.299682679)
( 0.0298364724, 0.281169727)
( 0.0323668929, 0.263491498)
( 0.0351119173, 0.246651473)
( 0.0380897464, 0.230646614)
( 0.041320124, 0.215468158)
( 0.0448244688, 0.201102386)
( 0.0486260158, 0.187531383)
( 0.0527499706, 0.174733743)
( 0.0572236766, 0.162685233)
( 0.0620767959, 0.151359399)
( 0.0673415066, 0.14072812)
( 0.0730527154, 0.130762093)
( 0.0792482898, 0.121431273)
( 0.0859693087, 0.112705246)
( 0.0932603347, 0.104553559)
( 0.10116971, 0.096945991)
( 0.109749877, 0.0898527851)
( 0.119057724, 0.0832448366)
( 0.129154967, 0.0770938451)
( 0.140108553, 0.071372433)
( 0.151991108, 0.066054235)
( 0.164881419, 0.0611139637)
( 0.178864953, 0.0565274517)
( 0.194034425, 0.052271677)
( 0.210490414, 0.0483247717)
( 0.22834203, 0.0446660188)
( 0.247707636, 0.0412758373)
( 0.268715631, 0.0381357598)
( 0.291505306, 0.0352284026)
( 0.316227766, 0.032537431)
};
\addplot [ black, dotted]
coordinates {
( 0.0001, 880.827036)
( 0.000108480964, 774.190152)
( 0.000117681195, 680.652505)
( 0.000127661695, 598.587681)
( 0.000138488637, 526.572739)
( 0.000150233808, 463.362627)
( 0.000162975083, 407.867829)
( 0.000176796941, 359.134822)
( 0.000191791026, 316.329005)
( 0.000208056754, 278.719772)
( 0.000225701972, 245.667473)
( 0.000244843675, 216.612013)
( 0.000265608778, 191.062885)
( 0.000288134963, 168.590461)
( 0.000312571585, 148.818376)
( 0.000339080668, 131.41687)
( 0.000367837977, 116.096964)
( 0.000399034183, 102.605375)
( 0.000432876128, 90.7200604)
( 0.000469588196, 80.2463257)
( 0.000509413801, 71.0134221)
( 0.000552617002, 62.8715668)
( 0.00059948425, 55.6893384)
( 0.000650326293, 49.351398)
( 0.000705480231, 43.7564954)
( 0.000765311755, 38.8157247)
( 0.000830217568, 34.4509977)
( 0.00090062802, 30.5937079)
( 0.000977009957, 27.1835613)
( 0.00105986982, 24.1675532)
( 0.001149757, 21.4990721)
( 0.00124726747, 19.1371156)
( 0.00135304777, 17.0456035)
( 0.00146779927, 15.1927769)
( 0.00159228279, 13.550671)
( 0.00172732372, 12.0946542)
( 0.00187381742, 10.8030241)
( 0.0020327352, 9.65665275)
( 0.00220513074, 8.63867683)
( 0.00239214708, 7.73422503)
( 0.00259502421, 6.93017943)
( 0.00281510728, 6.2149659)
( 0.00305385551, 5.57837013)
( 0.00331285189, 5.01137606)
( 0.00359381366, 4.50602372)
( 0.0038986037, 4.05528441)
( 0.00422924287, 3.65295068)
( 0.00458792343, 3.29353959)
( 0.00497702356, 2.97220735)
( 0.00539912314, 2.68467422)
( 0.00585702082, 2.42715815)
( 0.00635375264, 2.19631631)
( 0.0068926121, 1.98919347)
( 0.00747717205, 1.80317639)
( 0.00811130831, 1.63595368)
( 0.00879922544, 1.48548018)
( 0.00954548457, 1.34994569)
( 0.0103550337, 1.22774723)
( 0.0112332403, 1.1174647)
( 0.0121859274, 1.01783925)
( 0.0132194115, 0.927754337)
( 0.014340545, 0.846218974)
( 0.0155567614, 0.772352942)
( 0.0168761248, 0.705373808)
( 0.0183073828, 0.644585461)
( 0.0198600253, 0.589368035)
( 0.0215443469, 0.539169029)
( 0.0233715152, 0.493495498)
( 0.0253536449, 0.451907174)
( 0.0275038784, 0.414010422)
( 0.0298364724, 0.379452914)
( 0.0323668929, 0.347918941)
( 0.0351119173, 0.31912529)
( 0.0380897464, 0.292817612)
( 0.041320124, 0.268767214)
( 0.0448244688, 0.246768246)
( 0.0486260158, 0.226635205)
( 0.0527499706, 0.20820074)
( 0.0572236766, 0.191313709)
( 0.0620767959, 0.175837467)
( 0.0673415066, 0.161648342)
( 0.0730527154, 0.148634292)
( 0.0792482898, 0.136693711)
( 0.0859693087, 0.125734369)
( 0.0932603347, 0.115672471)
( 0.10116971, 0.106431816)
( 0.109749877, 0.0979430571)
( 0.119057724, 0.0901430256)
( 0.129154967, 0.0829741433)
( 0.140108553, 0.0763838864)
( 0.151991108, 0.0703243098)
( 0.164881419, 0.0647516192)
( 0.178864953, 0.0596257868)
( 0.194034425, 0.0549102068)
( 0.210490414, 0.0505713835)
( 0.22834203, 0.0465786524)
( 0.247707636, 0.0429039265)
( 0.268715631, 0.0395214683)
( 0.291505306, 0.0364076832)
( 0.316227766, 0.0335409328)
};
\addplot [blue, dashed]
coordinates {
( 0.02, 0.52263438)
( 0.3, 0.034842292)
};
\addplot [ red, dashed]
coordinates {
( 0.0001, 766.243411)
( 0.003, 2.64544048)
};
\addplot [ green, dashed]
coordinates {
( 0.002, 1)
( 0.3, 1)
};
\end{loglogaxis}


==> chiL.tex <==
\begin{loglogaxis}[
xmin= 0.1, xmax= 100,
ymin= 0.01, ymax= 10000,
xlabel={$|y|$},
ylabel={$\chi$},
ylabel near ticks,
grid
]
\addplot [black]
coordinates {
( 0.1, 0.999938516)
( 0.107226722, 0.99992857)
( 0.1149757, 0.999916898)
( 0.123284674, 0.999903168)
( 0.132194115, 0.999886977)
( 0.141747416, 0.999867825)
( 0.151991108, 0.999845105)
( 0.162975083, 0.999818063)
( 0.17475284, 0.999785768)
( 0.187381742, 0.999747063)
( 0.2009233, 0.999700507)
( 0.215443469, 0.999644303)
( 0.23101297, 0.999576202)
( 0.247707636, 0.99949339)
( 0.265608778, 0.999392339)
( 0.284803587, 0.99926863)
( 0.305385551, 0.999116728)
( 0.327454916, 0.998929712)
( 0.351119173, 0.998698942)
( 0.376493581, 0.998413675)
( 0.403701726, 0.998060591)
( 0.432876128, 0.997623264)
( 0.464158883, 0.997081555)
( 0.497702356, 0.996410935)
( 0.533669923, 0.995581776)
( 0.572236766, 0.994558614)
( 0.613590727, 0.993299442)
( 0.657933225, 0.991755085)
( 0.705480231, 0.989868734)
( 0.756463328, 0.987575718)
( 0.811130831, 0.984803605)
( 0.869749003, 0.981472723)
( 0.932603347, 0.977497176)
( 1, 0.97278639)
( 1.07226722, 0.967247215)
( 1.149757, 0.960786527)
( 1.23284674, 0.953314242)
( 1.32194115, 0.9447466)
( 1.41747416, 0.93500953)
( 1.51991108, 0.924041889)
( 1.62975083, 0.911798366)
( 1.7475284, 0.898251851)
( 1.87381742, 0.883395132)
( 2.009233, 0.867241798)
( 2.15443469, 0.849826323)
( 2.3101297, 0.831203351)
( 2.47707636, 0.811446247)
( 2.65608778, 0.790645034)
( 2.84803587, 0.768903864)
( 3.05385551, 0.746338173)
( 3.27454916, 0.723071681)
( 3.51119173, 0.699233374)
( 3.76493581, 0.674954603)
( 4.03701726, 0.650366391)
( 4.32876128, 0.625597027)
( 4.64158883, 0.600769992)
( 4.97702356, 0.576002244)
( 5.33669923, 0.551402872)
( 5.72236766, 0.52707209)
( 6.13590727, 0.503100569)
( 6.57933225, 0.479569062)
( 7.05480231, 0.45654829)
( 7.56463328, 0.434099039)
( 8.11130831, 0.412272451)
( 8.69749003, 0.391110445)
( 9.32603347, 0.370646254)
( 10, 0.350905032)
( 10.7226722, 0.331904519)
( 11.49757, 0.313655718)
( 12.3284674, 0.296163594)
( 13.2194115, 0.279427752)
( 14.1747416, 0.263443096)
( 15.1991108, 0.248200462)
( 16.2975083, 0.233687212)
( 17.475284, 0.219887779)
( 18.7381742, 0.206784179)
( 20.09233, 0.194356468)
( 21.5443469, 0.182583162)
( 23.101297, 0.171441608)
( 24.7707636, 0.160908313)
( 26.5608778, 0.150959236)
( 28.4803587, 0.141570038)
( 30.5385551, 0.132716305)
( 32.7454916, 0.124373728)
( 35.1119173, 0.116518266)
( 37.6493581, 0.109126277)
( 40.3701726, 0.102174623)
( 43.2876128, 0.0956407615)
( 46.4158883, 0.0895028136)
( 49.7702356, 0.0837396173)
( 53.3669923, 0.0783307668)
( 57.2236766, 0.07325664)
( 61.3590727, 0.0684984156)
( 65.7933225, 0.0640380806)
( 70.5480231, 0.0598584312)
( 75.6463328, 0.0559430667)
( 81.1130831, 0.0522763785)
( 86.9749003, 0.0488435352)
( 93.2603347, 0.0456304632)
( 100, 0.0426238259)
};
\addplot [ blue, dashed]
coordinates {
( 0.1, 2031597.07)
( 0.107226722, 1436308.06)
( 0.1149757, 1015768.51)
( 0.123284674, 718619.664)
( 0.132194115, 508608.481)
( 0.141747416, 360142.552)
( 0.151991108, 255153.47)
( 0.162975083, 180883.406)
( 0.17475284, 128323.106)
( 0.187381742, 91109.5262)
( 0.2009233, 64747.8371)
( 0.215443469, 46062.2934)
( 0.23101297, 32808.6323)
( 0.247707636, 23400.4577)
( 0.265608778, 16716.0729)
( 0.284803587, 11962.0944)
( 0.305385551, 8577.14317)
( 0.327454916, 6163.82905)
( 0.351119173, 4440.70681)
( 0.376493581, 3208.33458)
( 0.403701726, 2325.28968)
( 0.432876128, 1691.2166)
( 0.464158883, 1234.84215)
( 0.497702356, 905.499473)
( 0.533669923, 667.131646)
( 0.572236766, 494.047574)
( 0.613590727, 367.916803)
( 0.657933225, 275.640395)
( 0.705480231, 207.841574)
( 0.756463328, 157.794984)
( 0.811130831, 120.666485)
( 0.869749003, 92.9729527)
( 0.932603347, 72.1980089)
( 1, 56.5183592)
( 1.07226722, 44.6086475)
( 1.149757, 35.5020929)
( 1.23284674, 28.4907998)
( 1.32194115, 23.0543147)
( 1.41747416, 18.8083214)
( 1.51991108, 15.467712)
( 1.62975083, 12.8199395)
( 1.7475284, 10.705736)
( 1.87381742, 9.00511712)
( 2.009233, 7.62719149)
( 2.15443469, 6.5027135)
( 2.3101297, 5.57862049)
( 2.47707636, 4.81400965)
( 2.65608778, 4.17716235)
( 2.84803587, 3.64333365)
( 3.05385551, 3.19310247)
( 3.27454916, 2.81113443)
( 3.51119173, 2.48524958)
( 3.76493581, 2.2057163)
( 4.03701726, 1.96471387)
( 4.32876128, 1.75592119)
( 4.64158883, 1.57420059)
( 4.97702356, 1.41535329)
( 5.33669923, 1.27592942)
( 5.72236766, 1.15307961)
( 6.13590727, 1.04443852)
( 6.57933225, 0.948032924)
( 7.05480231, 0.862208769)
( 7.56463328, 0.785573149)
( 8.11130831, 0.716947776)
( 8.69749003, 0.655331578)
( 9.32603347, 0.599870463)
( 10, 0.549832778)
( 10.7226722, 0.504589294)
( 11.49757, 0.463596816)
( 12.3284674, 0.426384712)
( 13.2194115, 0.392543779)
( 14.1747416, 0.36171702)
( 15.1991108, 0.333591967)
( 16.2975083, 0.30789427)
( 17.475284, 0.284382317)
( 18.7381742, 0.262842711)
( 20.09233, 0.243086451)
( 21.5443469, 0.224945694)
( 23.101297, 0.208271007)
( 24.7707636, 0.192929021)
( 26.5608778, 0.178800421)
( 28.4803587, 0.16577823)
( 30.5385551, 0.153766325)
( 32.7454916, 0.142678157)
( 35.1119173, 0.132435646)
( 37.6493581, 0.122968225)
( 40.3701726, 0.114211997)
( 43.2876128, 0.106109009)
( 46.4158883, 0.0986066195)
( 49.7702356, 0.0916569305)
( 53.3669923, 0.0852163028)
( 57.2236766, 0.0792449202)
( 61.3590727, 0.0737064078)
( 65.7933225, 0.0685674932)
( 70.5480231, 0.0637977068)
( 75.6463328, 0.0593691141)
( 81.1130831, 0.0552560788)
( 86.9749003, 0.0514350501)
( 93.2603347, 0.047884373)
( 100, 0.0445841179)
};
\end{loglogaxis}


==> spectrum.tex <==
\begin{axis}[
xmin= 0, xmax= 1,
ymin= 0, ymax= 30,
xlabel={$\omega/\omega_{\rm cut}$},
ylabel={$\d\Sigma$},
ylabel near ticks,
]
\addplot []
coordinates {
( 1e-6, 50.605388)
( 0.00505149999, 24.9523027)
( 0.010102, 22.8128608)
( 0.0151525, 21.5402078)
( 0.020203, 20.6234053)
( 0.0252535, 19.9020893)
( 0.030304, 19.304731)
( 0.0353545, 18.7931242)
( 0.040405, 18.3444334)
( 0.0454555, 17.9439102)
( 0.0505059999, 17.5814714)
( 0.0555564999, 17.2499161)
( 0.0606069999, 16.9439205)
( 0.0656574999, 16.6594364)
( 0.0707079999, 16.3933132)
( 0.0757584999, 16.14305)
( 0.0808089999, 15.9066281)
( 0.0858594999, 15.6823943)
( 0.0909099999, 15.4689773)
( 0.0959604999, 15.265227)
( 0.101011, 15.070169)
( 0.1060615, 14.8829707)
( 0.111112, 14.7029148)
( 0.1161625, 14.5293787)
( 0.121213, 14.3618188)
( 0.1262635, 14.1997575)
( 0.131314, 14.0427727)
( 0.1363645, 13.8904896)
( 0.141415, 13.7425741)
( 0.1464655, 13.5987265)
( 0.151516, 13.4586774)
( 0.1565665, 13.3221837)
( 0.161617, 13.1890249)
( 0.1666675, 13.0590007)
( 0.171718, 12.9319284)
( 0.1767685, 12.8076412)
( 0.181819, 12.6859857)
( 0.1868695, 12.5668213)
( 0.19192, 12.4500184)
( 0.1969705, 12.335457)
( 0.202021, 12.2230265)
( 0.2070715, 12.1126239)
( 0.212122, 12.0041538)
( 0.2171725, 11.8975272)
( 0.222223, 11.7926612)
( 0.2272735, 11.6894783)
( 0.232324, 11.5879059)
( 0.2373745, 11.4878762)
( 0.242425, 11.3893254)
( 0.2474755, 11.2921934)
( 0.252526, 11.1964239)
( 0.2575765, 11.1019637)
( 0.262627, 11.0087626)
( 0.2676775, 10.9167731)
( 0.272728, 10.8259504)
( 0.2777785, 10.736252)
( 0.282829, 10.6476377)
( 0.2878795, 10.5600691)
( 0.29293, 10.4735099)
( 0.2979805, 10.3879257)
( 0.303031, 10.3032834)
( 0.3080815, 10.2195517)
( 0.313132, 10.1367008)
( 0.3181825, 10.054702)
( 0.323233, 9.97352812)
( 0.3282835, 9.89315298)
( 0.333334, 9.81355163)
( 0.3383845, 9.73470011)
( 0.343435, 9.65657549)
( 0.3484855, 9.57915574)
( 0.353536, 9.5024197)
( 0.3585865, 9.42634704)
( 0.363637, 9.35091821)
( 0.3686875, 9.27611438)
( 0.373738, 9.20191742)
( 0.3787885, 9.12830985)
( 0.383839, 9.0552748)
( 0.3888895, 8.982796)
( 0.39394, 8.91085772)
( 0.3989905, 8.83944474)
( 0.404041, 8.76854235)
( 0.4090915, 8.69813632)
( 0.414142, 8.62821284)
( 0.4191925, 8.55875852)
( 0.424243, 8.4897604)
( 0.4292935, 8.42120585)
( 0.434344, 8.35308265)
( 0.4393945, 8.28537888)
( 0.444445, 8.21808296)
( 0.4494955, 8.1511836)
( 0.454546, 8.08466983)
( 0.4595965, 8.01853092)
( 0.464647, 7.95275643)
( 0.4696975, 7.88733614)
( 0.474748, 7.82226007)
( 0.4797985, 7.75751848)
( 0.484849, 7.69310181)
( 0.4898995, 7.62900072)
( 0.49495, 7.56520604)
( 0.5000005, 7.50170878)
( 0.505050999, 7.43850012)
( 0.510101499, 7.37557139)
( 0.515151999, 7.31291405)
( 0.520202499, 7.25051973)
( 0.525252999, 7.18838016)
( 0.530303499, 7.12648719)
( 0.535353999, 7.06483279)
( 0.540404499, 7.00340902)
( 0.545454999, 6.94220804)
( 0.550505499, 6.88122209)
( 0.555555999, 6.82044348)
( 0.560606499, 6.7598646)
( 0.565656999, 6.69947789)
( 0.570707499, 6.63927585)
( 0.575757999, 6.57925102)
( 0.580808499, 6.51939599)
( 0.585858999, 6.45970335)
( 0.590909499, 6.40016574)
( 0.595959999, 6.3407758)
( 0.601010499, 6.28152617)
( 0.606060999, 6.22240952)
( 0.611111499, 6.16341846)
( 0.616161999, 6.10454561)
( 0.621212499, 6.04578357)
( 0.626262999, 5.98712489)
( 0.631313499, 5.92856207)
( 0.636363999, 5.87008757)
( 0.641414499, 5.81169377)
( 0.646464999, 5.753373)
( 0.651515499, 5.69511749)
( 0.656565999, 5.63691937)
( 0.661616499, 5.57877067)
( 0.666666999, 5.52066331)
( 0.671717499, 5.46258908)
( 0.676767999, 5.40453961)
( 0.681818499, 5.34650639)
( 0.686868999, 5.28848073)
( 0.691919499, 5.23045376)
( 0.696969999, 5.17241641)
( 0.702020499, 5.11435939)
( 0.707070999, 5.05627316)
( 0.712121499, 4.99814793)
( 0.717171999, 4.93997363)
( 0.722222499, 4.88173989)
( 0.727272999, 4.82343602)
( 0.732323499, 4.76505097)
( 0.737373999, 4.7065733)
( 0.742424499, 4.64799118)
( 0.747474999, 4.58929232)
( 0.752525499, 4.53046395)
( 0.757575999, 4.47149278)
( 0.762626499, 4.41236495)
( 0.767676999, 4.35306602)
( 0.772727499, 4.29358084)
( 0.777777999, 4.23389357)
( 0.782828499, 4.17398758)
( 0.787878999, 4.1138454)
( 0.792929499, 4.0534486)
( 0.797979999, 3.99277777)
( 0.803030499, 3.93181237)
( 0.808080999, 3.87053066)
( 0.813131499, 3.80890956)
( 0.818181999, 3.74692452)
( 0.823232499, 3.6845494)
( 0.828282999, 3.62175624)
( 0.833333499, 3.55851514)
( 0.838383999, 3.49479398)
( 0.843434499, 3.43055822)
( 0.848484999, 3.36577058)
( 0.853535499, 3.30039073)
( 0.858585999, 3.23437489)
( 0.863636499, 3.16767541)
( 0.868686999, 3.10024025)
( 0.873737499, 3.03201235)
( 0.878787999, 2.96292893)
( 0.883838499, 2.89292061)
( 0.888888999, 2.82191041)
( 0.893939499, 2.74981248)
( 0.898989999, 2.67653062)
( 0.904040499, 2.60195637)
( 0.909090999, 2.52596673)
( 0.914141499, 2.44842125)
( 0.919191999, 2.36915835)
( 0.924242499, 2.28799057)
( 0.929292999, 2.20469833)
( 0.934343499, 2.11902174)
( 0.939393999, 2.03064935)
( 0.944444499, 1.93920268)
( 0.949494999, 1.84421414)
( 0.954545499, 1.74509471)
( 0.959595999, 1.64108483)
( 0.964646499, 1.53117633)
( 0.969696999, 1.41398172)
( 0.974747499, 1.2874992)
( 0.979797999, 1.14864953)
( 0.984848499, 0.992237205)
( 0.989898999, 0.808107157)
( 0.994949499, 0.569973619)
( 0.999999999, 0.000252982841)
};
\addplot [blue, dashed]
coordinates {
( 0.65, 6.80145044)
( 0.653535354, 6.77865648)
( 0.657070707, 6.75575764)
( 0.660606061, 6.73275244)
( 0.664141414, 6.70963942)
( 0.667676768, 6.68641705)
( 0.671212121, 6.66308378)
( 0.674747475, 6.63963802)
( 0.678282828, 6.61607814)
( 0.681818182, 6.59240247)
( 0.685353535, 6.5686093)
( 0.688888889, 6.54469689)
( 0.692424242, 6.52066343)
( 0.695959596, 6.49650709)
( 0.699494949, 6.47222598)
( 0.703030303, 6.44781818)
( 0.706565656, 6.42328169)
( 0.71010101, 6.39861449)
( 0.713636363, 6.37381448)
( 0.717171717, 6.34887952)
( 0.720707071, 6.32380741)
( 0.724242424, 6.29859588)
( 0.727777778, 6.27324262)
( 0.731313131, 6.24774525)
( 0.734848485, 6.22210129)
( 0.738383838, 6.19630824)
( 0.741919192, 6.1703635)
( 0.745454545, 6.14426439)
( 0.748989899, 6.11800818)
( 0.752525252, 6.09159204)
( 0.756060606, 6.06501304)
( 0.759595959, 6.0382682)
( 0.763131313, 6.01135442)
( 0.766666666, 5.98426852)
( 0.77020202, 5.95700721)
( 0.773737373, 5.9295671)
( 0.777272727, 5.90194471)
( 0.78080808, 5.87413642)
( 0.784343434, 5.8461385)
( 0.787878787, 5.81794711)
( 0.791414141, 5.78955828)
( 0.794949495, 5.7609679)
( 0.798484848, 5.73217172)
( 0.802020202, 5.70316534)
( 0.805555555, 5.67394422)
( 0.809090909, 5.64450365)
( 0.812626262, 5.61483876)
( 0.816161616, 5.58494449)
( 0.819696969, 5.55481563)
( 0.823232323, 5.52444674)
( 0.826767676, 5.49383219)
( 0.83030303, 5.46296616)
( 0.833838383, 5.43184258)
( 0.837373737, 5.40045516)
( 0.84090909, 5.36879737)
( 0.844444444, 5.33686242)
( 0.847979797, 5.30464326)
( 0.851515151, 5.27213256)
( 0.855050504, 5.23932268)
( 0.858585858, 5.20620569)
( 0.862121212, 5.17277335)
( 0.865656565, 5.13901706)
( 0.869191919, 5.10492789)
( 0.872727272, 5.07049654)
( 0.876262626, 5.03571333)
( 0.879797979, 5.00056821)
( 0.883333333, 4.96505071)
( 0.886868686, 4.92914996)
( 0.89040404, 4.89285467)
( 0.893939393, 4.85615313)
( 0.897474747, 4.81903322)
( 0.9010101, 4.7814824)
( 0.904545454, 4.74348778)
( 0.908080807, 4.70503607)
( 0.911616161, 4.66611374)
( 0.915151514, 4.626707)
( 0.918686868, 4.58680199)
( 0.922222221, 4.5463849)
( 0.925757575, 4.5054422)
( 0.929292928, 4.46396099)
( 0.932828282, 4.42192937)
( 0.936363636, 4.37933712)
( 0.939898989, 4.33617644)
( 0.943434343, 4.29244322)
( 0.946969696, 4.24813858)
( 0.95050505, 4.20327126)
( 0.954040403, 4.15786089)
( 0.957575757, 4.11194283)
( 0.96111111, 4.06557528)
( 0.964646464, 4.01884984)
( 0.968181817, 3.9719078)
( 0.971717171, 3.92496549)
( 0.975252524, 3.87835495)
( 0.978787878, 3.83259098)
( 0.982323231, 3.78848494)
( 0.985858585, 3.74734183)
( 0.989393938, 3.71129979)
( 0.992929292, 3.68383325)
( 0.996464645, 3.66969251)
( 0.999999999, 3.66804948)
};
\addplot [blue, dashed]
coordinates {
( 0.65, 3.13340096)
( 0.653535354, 3.11060701)
( 0.657070707, 3.08770816)
( 0.660606061, 3.06470297)
( 0.664141414, 3.04158995)
( 0.667676768, 3.01836758)
( 0.671212121, 2.99503431)
( 0.674747475, 2.97158855)
( 0.678282828, 2.94802866)
( 0.681818182, 2.92435299)
( 0.685353535, 2.90055983)
( 0.688888889, 2.87664741)
( 0.692424242, 2.85261395)
( 0.695959596, 2.82845761)
( 0.699494949, 2.80417651)
( 0.703030303, 2.77976871)
( 0.706565656, 2.75523222)
( 0.71010101, 2.73056501)
( 0.713636363, 2.705765)
( 0.717171717, 2.68083004)
( 0.720707071, 2.65575793)
( 0.724242424, 2.63054641)
( 0.727777778, 2.60519315)
( 0.731313131, 2.57969577)
( 0.734848485, 2.55405182)
( 0.738383838, 2.52825876)
( 0.741919192, 2.50231402)
( 0.745454545, 2.47621492)
( 0.748989899, 2.44995871)
( 0.752525252, 2.42354256)
( 0.756060606, 2.39696357)
( 0.759595959, 2.37021872)
( 0.763131313, 2.34330494)
( 0.766666666, 2.31621904)
( 0.77020202, 2.28895773)
( 0.773737373, 2.26151763)
( 0.777272727, 2.23389523)
( 0.78080808, 2.20608694)
( 0.784343434, 2.17808902)
( 0.787878787, 2.14989764)
( 0.791414141, 2.12150881)
( 0.794949495, 2.09291842)
( 0.798484848, 2.06412224)
( 0.802020202, 2.03511586)
( 0.805555555, 2.00589474)
( 0.809090909, 1.97645417)
( 0.812626262, 1.94678928)
( 0.816161616, 1.91689502)
( 0.819696969, 1.88676615)
( 0.823232323, 1.85639726)
( 0.826767676, 1.82578272)
( 0.83030303, 1.79491668)
( 0.833838383, 1.7637931)
( 0.837373737, 1.73240568)
( 0.84090909, 1.70074789)
( 0.844444444, 1.66881295)
( 0.847979797, 1.63659379)
( 0.851515151, 1.60408308)
( 0.855050504, 1.5712732)
( 0.858585858, 1.53815622)
( 0.862121212, 1.50472387)
( 0.865656565, 1.47096758)
( 0.869191919, 1.43687841)
( 0.872727272, 1.40244706)
( 0.876262626, 1.36766386)
( 0.879797979, 1.33251874)
( 0.883333333, 1.29700124)
( 0.886868686, 1.26110049)
( 0.89040404, 1.22480519)
( 0.893939393, 1.18810365)
( 0.897474747, 1.15098374)
( 0.9010101, 1.11343293)
( 0.904545454, 1.0754383)
( 0.908080807, 1.0369866)
( 0.911616161, 0.998064263)
( 0.915151514, 0.958657525)
( 0.918686868, 0.918752514)
( 0.922222221, 0.87833542)
( 0.925757575, 0.837392726)
( 0.929292928, 0.795911513)
( 0.932828282, 0.753879899)
( 0.936363636, 0.711287642)
( 0.939898989, 0.668126968)
( 0.943434343, 0.624393743)
( 0.946969696, 0.580089105)
( 0.95050505, 0.535221781)
( 0.954040403, 0.48981141)
( 0.957575757, 0.443893356)
( 0.96111111, 0.397525802)
( 0.964646464, 0.350800364)
( 0.968181817, 0.303858329)
( 0.971717171, 0.256916018)
( 0.975252524, 0.210305471)
( 0.978787878, 0.164541508)
( 0.982323231, 0.120435464)
( 0.985858585, 0.0792923561)
( 0.989393938, 0.0432503135)
( 0.992929292, 0.0157837708)
( 0.996464645, 0.00164303212)
( 0.999999999, 0)
};
\addplot [red, dash dot]
coordinates {
( 0.8, 4.22380378)
( 0.802020202, 4.20586486)
( 0.804040404, 4.18783598)
( 0.806060606, 4.16971577)
( 0.808080808, 4.15150285)
( 0.81010101, 4.13319576)
( 0.812121212, 4.11479303)
( 0.814141414, 4.09629316)
( 0.816161616, 4.07769457)
( 0.818181818, 4.05899569)
( 0.82020202, 4.04019486)
( 0.822222222, 4.02129041)
( 0.824242424, 4.00228059)
( 0.826262626, 3.98316363)
( 0.828282828, 3.96393771)
( 0.83030303, 3.94460092)
( 0.832323232, 3.92515134)
( 0.834343434, 3.90558697)
( 0.836363636, 3.88590574)
( 0.838383838, 3.86610555)
( 0.84040404, 3.84618421)
( 0.842424242, 3.82613947)
( 0.844444444, 3.80596901)
( 0.846464646, 3.78567043)
( 0.848484848, 3.76524126)
( 0.85050505, 3.74467895)
( 0.852525252, 3.72398086)
( 0.854545454, 3.70314428)
( 0.856565656, 3.68216637)
( 0.858585858, 3.66104423)
( 0.86060606, 3.63977485)
( 0.862626262, 3.61835509)
( 0.864646464, 3.59678174)
( 0.866666666, 3.57505143)
( 0.868686868, 3.5531607)
( 0.87070707, 3.53110593)
( 0.872727272, 3.50888339)
( 0.874747474, 3.48648919)
( 0.876767676, 3.46391929)
( 0.878787878, 3.4411695)
( 0.88080808, 3.41823544)
( 0.882828282, 3.39511258)
( 0.884848484, 3.37179616)
( 0.886868686, 3.34828125)
( 0.888888888, 3.32456269)
( 0.89090909, 3.30063512)
( 0.892929292, 3.2764929)
( 0.894949494, 3.25213015)
( 0.896969696, 3.22754074)
( 0.898989898, 3.20271821)
( 0.901010101, 3.17765582)
( 0.903030303, 3.15234648)
( 0.905050505, 3.12678275)
( 0.907070707, 3.10095682)
( 0.909090909, 3.07486045)
( 0.911111111, 3.04848497)
( 0.913131313, 3.02182125)
( 0.915151515, 2.99485964)
( 0.917171717, 2.96758994)
( 0.919191919, 2.94000135)
( 0.921212121, 2.91208245)
( 0.923232323, 2.88382108)
( 0.925252525, 2.85520435)
( 0.927272727, 2.82621854)
( 0.929292929, 2.79684901)
( 0.931313131, 2.76708014)
( 0.933333333, 2.73689521)
( 0.935353535, 2.70627634)
( 0.937373737, 2.67520428)
( 0.939393939, 2.64365835)
( 0.941414141, 2.61161626)
( 0.943434343, 2.5790539)
( 0.945454545, 2.54594516)
( 0.947474747, 2.51226167)
( 0.949494949, 2.47797255)
( 0.951515151, 2.44304404)
( 0.953535353, 2.40743915)
( 0.955555555, 2.3711172)
( 0.957575757, 2.33403329)
( 0.959595959, 2.29613766)
( 0.961616161, 2.25737492)
( 0.963636363, 2.21768317)
( 0.965656565, 2.17699282)
( 0.967676767, 2.13522526)
( 0.969696969, 2.09229111)
( 0.971717171, 2.04808815)
( 0.973737373, 2.00249856)
( 0.975757575, 1.95538553)
( 0.977777777, 1.90658882)
( 0.979797979, 1.85591905)
( 0.981818181, 1.80315012)
( 0.983838383, 1.7480095)
( 0.985858585, 1.69016554)
( 0.987878787, 1.62921227)
( 0.989898989, 1.56465471)
( 0.991919191, 1.49591043)
( 0.993939393, 1.42239867)
( 0.995959595, 1.3440765)
( 0.997979797, 1.26488066)
( 0.999999999, 1.22268316)
};
\addplot [red, dash dot]
coordinates {
( 0.8, 3.00112062)
( 0.802020202, 2.9831817)
( 0.804040404, 2.96515282)
( 0.806060606, 2.94703261)
( 0.808080808, 2.92881969)
( 0.81010101, 2.9105126)
( 0.812121212, 2.89210987)
( 0.814141414, 2.87361)
( 0.816161616, 2.85501141)
( 0.818181818, 2.83631253)
( 0.82020202, 2.8175117)
( 0.822222222, 2.79860725)
( 0.824242424, 2.77959743)
( 0.826262626, 2.76048048)
( 0.828282828, 2.74125455)
( 0.83030303, 2.72191776)
( 0.832323232, 2.70246818)
( 0.834343434, 2.68290381)
( 0.836363636, 2.66322258)
( 0.838383838, 2.64342239)
( 0.84040404, 2.62350105)
( 0.842424242, 2.60345631)
( 0.844444444, 2.58328585)
( 0.846464646, 2.56298727)
( 0.848484848, 2.5425581)
( 0.85050505, 2.52199579)
( 0.852525252, 2.50129771)
( 0.854545454, 2.48046112)
( 0.856565656, 2.45948321)
( 0.858585858, 2.43836107)
( 0.86060606, 2.41709169)
( 0.862626262, 2.39567194)
( 0.864646464, 2.37409858)
( 0.866666666, 2.35236827)
( 0.868686868, 2.33047754)
( 0.87070707, 2.30842277)
( 0.872727272, 2.28620023)
( 0.874747474, 2.26380603)
( 0.876767676, 2.24123613)
( 0.878787878, 2.21848634)
( 0.88080808, 2.19555229)
( 0.882828282, 2.17242942)
( 0.884848484, 2.149113)
( 0.886868686, 2.12559809)
( 0.888888888, 2.10187954)
( 0.89090909, 2.07795196)
( 0.892929292, 2.05380974)
( 0.894949494, 2.029447)
( 0.896969696, 2.00485758)
( 0.898989898, 1.98003505)
( 0.901010101, 1.95497266)
( 0.903030303, 1.92966332)
( 0.905050505, 1.90409959)
( 0.907070707, 1.87827366)
( 0.909090909, 1.85217729)
( 0.911111111, 1.82580181)
( 0.913131313, 1.79913809)
( 0.915151515, 1.77217648)
( 0.917171717, 1.74490678)
( 0.919191919, 1.7173182)
( 0.921212121, 1.68939929)
( 0.923232323, 1.66113792)
( 0.925252525, 1.63252119)
( 0.927272727, 1.60353538)
( 0.929292929, 1.57416585)
( 0.931313131, 1.54439698)
( 0.933333333, 1.51421206)
( 0.935353535, 1.48359318)
( 0.937373737, 1.45252112)
( 0.939393939, 1.42097519)
( 0.941414141, 1.3889331)
( 0.943434343, 1.35637074)
( 0.945454545, 1.323262)
( 0.947474747, 1.28957851)
( 0.949494949, 1.25528939)
( 0.951515151, 1.22036088)
( 0.953535353, 1.18475599)
( 0.955555555, 1.14843404)
( 0.957575757, 1.11135013)
( 0.959595959, 1.0734545)
( 0.961616161, 1.03469176)
( 0.963636363, 0.995000014)
( 0.965656565, 0.954309665)
( 0.967676767, 0.912542099)
( 0.969696969, 0.869607954)
( 0.971717171, 0.825404991)
( 0.973737373, 0.7798154)
( 0.975757575, 0.73270237)
( 0.977777777, 0.683905666)
( 0.979797979, 0.633235887)
( 0.981818181, 0.580466961)
( 0.983838383, 0.525326338)
( 0.985858585, 0.467482379)
( 0.987878787, 0.406529116)
( 0.989898989, 0.341971547)
( 0.991919191, 0.273227273)
( 0.993939393, 0.199715507)
( 0.995959595, 0.12139334)
( 0.997979797, 0.0421975017)
( 0.999999999, 0)
};
\end{axis}


==> spectrum_log.tex <==
\begin{loglogaxis}[
xmin= 0.01, xmax= 1,
ymin= 0.01, ymax= 100,
xlabel={$x$},
ylabel={$\d\Sigma$},
ylabel near ticks,
]
\addplot []
coordinates {
( 0.01, 0.0800040002)
( 0.0100927105, 0.0807457964)
( 0.0101862805, 0.0814944719)
( 0.010280718, 0.0822500906)
( 0.010376031, 0.083012717)
( 0.0104722277, 0.083782416)
( 0.0105693163, 0.0845592532)
( 0.0106673049, 0.085343295)
( 0.010766202, 0.0861346081)
( 0.010866016, 0.0869332602)
( 0.0109667554, 0.0877393192)
( 0.0110684287, 0.0885528539)
( 0.0111710446, 0.0893739337)
( 0.0112746119, 0.0902026287)
( 0.0113791394, 0.0910390094)
( 0.011484636, 0.0918831474)
( 0.0115911106, 0.0927351144)
( 0.0116985724, 0.0935949833)
( 0.0118070304, 0.0944628274)
( 0.011916494, 0.0953387207)
( 0.0120269724, 0.0962227379)
( 0.012138475, 0.0971149545)
( 0.0122510114, 0.0980154465)
( 0.0123645911, 0.0989242908)
( 0.0124792239, 0.0998415649)
( 0.0125949193, 0.100767347)
( 0.0127116875, 0.101701716)
( 0.0128295381, 0.102644752)
( 0.0129484814, 0.103596536)
( 0.0130685274, 0.104557148)
( 0.0131896864, 0.10552667)
( 0.0133119686, 0.106505185)
( 0.0134353845, 0.107492778)
( 0.0135599446, 0.108489531)
( 0.0136856595, 0.10949553)
( 0.0138125399, 0.110510861)
( 0.0139405967, 0.111535611)
( 0.0140698406, 0.112569867)
( 0.0142002828, 0.113613717)
( 0.0143319343, 0.114667251)
( 0.0144648064, 0.115730558)
( 0.0145989103, 0.116803729)
( 0.0147342575, 0.117886857)
( 0.0148708596, 0.118980032)
( 0.015008728, 0.120083349)
( 0.0151478747, 0.121196902)
( 0.0152883114, 0.122320786)
( 0.01543005, 0.123455097)
( 0.0155731028, 0.124599931)
( 0.0157174818, 0.125755387)
( 0.0158631993, 0.126921564)
( 0.0160102678, 0.12809856)
( 0.0161586998, 0.129286477)
( 0.0163085079, 0.130485415)
( 0.0164597049, 0.131695478)
( 0.0166123036, 0.132916769)
( 0.0167663171, 0.134149391)
( 0.0169217584, 0.135393452)
( 0.0170786409, 0.136649055)
( 0.0172369778, 0.13791631)
( 0.0173967827, 0.139195324)
( 0.0175580691, 0.140486207)
( 0.0177208508, 0.141789069)
( 0.0178851417, 0.143104021)
( 0.0180509557, 0.144431175)
( 0.018218307, 0.145770646)
( 0.0183872098, 0.147122548)
( 0.0185576785, 0.148486996)
( 0.0187297277, 0.149864107)
( 0.0189033719, 0.151253999)
( 0.019078626, 0.15265679)
( 0.0192555049, 0.154072601)
( 0.0194340236, 0.155501553)
( 0.0196141974, 0.156943767)
( 0.0197960416, 0.158399368)
( 0.0199795716, 0.15986848)
( 0.0201648032, 0.161351229)
( 0.0203517521, 0.162847741)
( 0.0205404342, 0.164358144)
( 0.0207308655, 0.165882568)
( 0.0209230624, 0.167421144)
( 0.0211170411, 0.168974003)
( 0.0213128183, 0.170541277)
( 0.0215104104, 0.172123102)
( 0.0217098345, 0.173719613)
( 0.0219111075, 0.175330946)
( 0.0221142464, 0.176957239)
( 0.0223192687, 0.178598632)
( 0.0225261917, 0.180255265)
( 0.0227350331, 0.18192728)
( 0.0229458107, 0.183614821)
( 0.0231585425, 0.185318032)
( 0.0233732464, 0.187037059)
( 0.0235899409, 0.188772049)
( 0.0238086444, 0.190523152)
( 0.0240293756, 0.192290517)
( 0.0242521531, 0.194074295)
( 0.024476996, 0.195874641)
( 0.0247039234, 0.197691707)
( 0.0249329547, 0.199525651)
( 0.0251641093, 0.20137663)
( 0.025397407, 0.203244801)
( 0.0256328676, 0.205130326)
( 0.0258705112, 0.207033367)
( 0.0261103579, 0.208954086)
( 0.0263524284, 0.210892649)
( 0.026596743, 0.212849222)
( 0.0268433227, 0.214823973)
( 0.0270921885, 0.216817072)
( 0.0273433615, 0.21882869)
( 0.0275968631, 0.220859)
( 0.027852715, 0.222908176)
( 0.0281109389, 0.224976395)
( 0.0283715568, 0.227063834)
( 0.0286345908, 0.229170672)
( 0.0289000635, 0.231297092)
( 0.0291679974, 0.233443275)
( 0.0294384154, 0.235609406)
( 0.0297113404, 0.237795672)
( 0.0299867957, 0.240002261)
( 0.0302648047, 0.242229363)
( 0.0305453912, 0.24447717)
( 0.030828579, 0.246745875)
( 0.0311143923, 0.249035673)
( 0.0314028553, 0.251346762)
( 0.0316939927, 0.253679341)
( 0.0319878293, 0.25603361)
( 0.03228439, 0.258409774)
( 0.0325837002, 0.260808036)
( 0.0328857852, 0.263228604)
( 0.033190671, 0.265671686)
( 0.0334983833, 0.268137494)
( 0.0338089485, 0.270626239)
( 0.0341223929, 0.273138137)
( 0.0344387432, 0.275673405)
( 0.0347580265, 0.278232261)
( 0.0350802699, 0.280814927)
( 0.0354055008, 0.283421626)
( 0.0357337469, 0.286052582)
( 0.0360650362, 0.288708025)
( 0.0363993969, 0.291388182)
( 0.0367368575, 0.294093287)
( 0.0370774467, 0.296823573)
( 0.0374211936, 0.299579276)
( 0.0377681273, 0.302360636)
( 0.0381182774, 0.305167892)
( 0.0384716738, 0.308001289)
( 0.0388283466, 0.310861071)
( 0.0391883261, 0.313747487)
( 0.039551643, 0.316660787)
( 0.0399183282, 0.319601223)
( 0.040288413, 0.322569051)
( 0.0406619288, 0.325564529)
( 0.0410389076, 0.328587917)
( 0.0414193813, 0.331639476)
( 0.0418033824, 0.334719473)
( 0.0421909436, 0.337828175)
( 0.0425820979, 0.340965853)
( 0.0429768786, 0.344132779)
( 0.0433753194, 0.347329229)
( 0.0437774541, 0.350555482)
( 0.044183317, 0.353811818)
( 0.0445929427, 0.357098522)
( 0.045006366, 0.360415879)
( 0.0454236222, 0.363764179)
( 0.0458447469, 0.367143715)
( 0.0462697758, 0.37055478)
( 0.0466987451, 0.373997674)
( 0.0471316915, 0.377472697)
( 0.0475686517, 0.380980153)
( 0.048009663, 0.384520348)
( 0.0484547629, 0.388093592)
( 0.0489039894, 0.391700199)
( 0.0493573807, 0.395340483)
( 0.0498149754, 0.399014764)
( 0.0502768124, 0.402723365)
( 0.0507429312, 0.40646661)
( 0.0512133714, 0.410244828)
( 0.0516881731, 0.41405835)
( 0.0521673767, 0.417907513)
( 0.052651023, 0.421792654)
( 0.0531391532, 0.425714116)
( 0.0536318089, 0.429672242)
( 0.054129032, 0.433667383)
( 0.0546308649, 0.437699889)
( 0.0551373503, 0.441770118)
( 0.0556485314, 0.445878427)
( 0.0561644516, 0.45002518)
( 0.056685155, 0.454210743)
( 0.0572106859, 0.458435486)
( 0.0577410889, 0.462699783)
( 0.0582764094, 0.467004012)
( 0.0588166928, 0.471348554)
( 0.0593619853, 0.475733794)
( 0.0599123331, 0.480160121)
( 0.0604677833, 0.484627929)
( 0.0610283831, 0.489137614)
( 0.0615941802, 0.493689578)
( 0.0621652229, 0.498284226)
( 0.0627415597, 0.502921967)
( 0.0633232398, 0.507603214)
( 0.0639103126, 0.512328385)
( 0.0645028282, 0.517097903)
( 0.0651008371, 0.521912193)
( 0.0657043902, 0.526771687)
( 0.0663135388, 0.531676819)
( 0.0669283348, 0.536628029)
( 0.0675488307, 0.541625762)
( 0.0681750792, 0.546670465)
( 0.0688071337, 0.551762593)
( 0.069445048, 0.556902603)
( 0.0700888765, 0.562090959)
( 0.0707386739, 0.567328128)
( 0.0713944956, 0.572614583)
( 0.0720563974, 0.577950801)
( 0.0727244358, 0.583337265)
( 0.0733986676, 0.588774463)
( 0.0740791503, 0.594262887)
( 0.0747659417, 0.599803035)
( 0.0754591004, 0.605395411)
( 0.0761586854, 0.611040524)
( 0.0768647563, 0.616738886)
( 0.0775773732, 0.622491019)
( 0.0782965968, 0.628297446)
( 0.0790224884, 0.634158698)
( 0.0797551098, 0.640075312)
( 0.0804945233, 0.64604783)
( 0.0812407919, 0.6520768)
( 0.0819939793, 0.658162776)
( 0.0827541495, 0.664306317)
( 0.0835213673, 0.67050799)
( 0.0842956979, 0.676768366)
( 0.0850772075, 0.683088025)
( 0.0858659624, 0.68946755)
( 0.08666203, 0.695907533)
( 0.0874654779, 0.702408571)
( 0.0882763746, 0.708971269)
( 0.0890947892, 0.715596237)
( 0.0899207913, 0.722284094)
( 0.0907544514, 0.729035463)
( 0.0915958404, 0.735850977)
( 0.0924450299, 0.742731273)
( 0.0933020923, 0.749676998)
( 0.0941671005, 0.756688805)
( 0.0950401283, 0.763767354)
( 0.09592125, 0.770913312)
( 0.0968105406, 0.778127356)
( 0.0977080759, 0.785410168)
( 0.0986139322, 0.79276244)
( 0.0995281868, 0.80018487)
( 0.100450917, 0.807678165)
( 0.101382203, 0.815243041)
( 0.102322122, 0.822880221)
( 0.103270756, 0.830590436)
( 0.104228184, 0.838374428)
( 0.105194488, 0.846232944)
( 0.106169752, 0.854166743)
( 0.107154057, 0.862176592)
( 0.108147487, 0.870263267)
( 0.109150128, 0.878427551)
( 0.110162064, 0.886670241)
( 0.111183382, 0.894992139)
( 0.112214168, 0.90339406)
( 0.113254511, 0.911876826)
( 0.1143045, 0.920441272)
( 0.115364222, 0.92908824)
( 0.11643377, 0.937818584)
( 0.117513233, 0.946633169)
( 0.118602704, 0.955532868)
( 0.119702275, 0.964518569)
( 0.120812041, 0.973591167)
( 0.121932095, 0.982751571)
( 0.123062533, 0.992000699)
( 0.124203452, 1.00133948)
( 0.125354949, 1.01076886)
( 0.12651712, 1.02028979)
( 0.127690067, 1.02990324)
( 0.128873888, 1.03961019)
( 0.130068684, 1.04941163)
( 0.131274557, 1.05930855)
( 0.13249161, 1.06930199)
( 0.133719946, 1.07939297)
( 0.13495967, 1.08958253)
( 0.136210888, 1.09987173)
( 0.137473706, 1.11026165)
( 0.138748231, 1.12075336)
( 0.140034573, 1.13134798)
( 0.14133284, 1.1420466)
( 0.142643144, 1.15285037)
( 0.143965595, 1.16376043)
( 0.145300307, 1.17477793)
( 0.146647394, 1.18590407)
( 0.148006969, 1.19714002)
( 0.149379149, 1.20848699)
( 0.15076405, 1.21994622)
( 0.152161791, 1.23151895)
( 0.15357249, 1.24320643)
( 0.154996268, 1.25500995)
( 0.156433246, 1.2669308)
( 0.157883547, 1.27897029)
( 0.159347293, 1.29112976)
( 0.160824609, 1.30341056)
( 0.162315622, 1.31581406)
( 0.163820458, 1.32834166)
( 0.165339246, 1.34099477)
( 0.166872114, 1.35377481)
( 0.168419193, 1.36668325)
( 0.169980616, 1.37972156)
( 0.171556515, 1.39289124)
( 0.173147023, 1.40619381)
( 0.174752278, 1.41963081)
( 0.176372415, 1.43320381)
( 0.178007572, 1.44691439)
( 0.179657889, 1.46076419)
( 0.181323506, 1.47475483)
( 0.183004565, 1.48888798)
( 0.18470121, 1.50316533)
( 0.186413583, 1.5175886)
( 0.188141833, 1.53215955)
( 0.189886105, 1.54687993)
( 0.191646548, 1.56175155)
( 0.193423313, 1.57677625)
( 0.19521655, 1.59195589)
( 0.197026412, 1.60729235)
( 0.198853054, 1.62278756)
( 0.20069663, 1.63844347)
( 0.202557298, 1.65426208)
( 0.204435217, 1.67024539)
( 0.206330546, 1.68639546)
( 0.208243446, 1.70271439)
( 0.210174082, 1.71920429)
( 0.212122616, 1.73586733)
( 0.214089215, 1.7527057)
( 0.216074047, 1.76972164)
( 0.21807728, 1.78691744)
( 0.220099085, 1.80429539)
( 0.222139634, 1.82185786)
( 0.224199101, 1.83960725)
( 0.226277662, 1.85754601)
( 0.228375494, 1.8756766)
( 0.230492774, 1.89400158)
( 0.232629684, 1.91252351)
( 0.234786405, 1.93124502)
( 0.236963121, 1.95016879)
( 0.239160018, 1.96929753)
( 0.241377282, 1.98863403)
( 0.243615103, 2.00818111)
( 0.24587367, 2.02794166)
( 0.248153177, 2.0479186)
( 0.250453817, 2.06811494)
( 0.252775787, 2.08853373)
( 0.255119284, 2.10917808)
( 0.257484507, 2.13005117)
( 0.259871658, 2.15115622)
( 0.262280941, 2.17249655)
( 0.264712561, 2.19407552)
( 0.267166724, 2.21589656)
( 0.269643639, 2.23796319)
( 0.272143519, 2.26027899)
( 0.274666575, 2.2828476)
( 0.277213022, 2.30567276)
( 0.279783077, 2.32875828)
( 0.28237696, 2.35210804)
( 0.284994891, 2.37572601)
( 0.287637092, 2.39961626)
( 0.29030379, 2.42378293)
( 0.29299521, 2.44823025)
( 0.295711583, 2.47296255)
( 0.29845314, 2.49798427)
( 0.301220114, 2.52329991)
( 0.30401274, 2.5489141)
( 0.306831257, 2.57483158)
( 0.309675905, 2.60105718)
( 0.312546925, 2.62759585)
( 0.315444563, 2.65445265)
( 0.318369065, 2.68163276)
( 0.32132068, 2.70914148)
( 0.32429966, 2.73698425)
( 0.327306258, 2.76516661)
( 0.33034073, 2.79369426)
( 0.333403335, 2.82257303)
( 0.336494334, 2.85180888)
( 0.339613989, 2.88140794)
( 0.342762567, 2.91137647)
( 0.345940336, 2.9417209)
( 0.349147565, 2.97244782)
( 0.35238453, 3.00356398)
( 0.355651504, 3.0350763)
( 0.358948766, 3.0669919)
( 0.362276598, 3.09931806)
( 0.365635282, 3.13206227)
( 0.369025104, 3.16523221)
( 0.372446354, 3.19883576)
( 0.375899323, 3.23288101)
( 0.379384304, 3.26737629)
( 0.382901594, 3.30233013)
( 0.386451493, 3.33775132)
( 0.390034304, 3.37364888)
( 0.393650331, 3.41003207)
( 0.397299883, 3.44691045)
( 0.400983269, 3.48429382)
( 0.404700805, 3.52219227)
( 0.408452806, 3.5606162)
( 0.412239592, 3.59957628)
( 0.416061485, 3.63908354)
( 0.419918812, 3.6791493)
( 0.423811899, 3.71978524)
( 0.42774108, 3.7610034)
( 0.431706689, 3.80281618)
( 0.435709063, 3.84523636)
( 0.439748543, 3.88827715)
( 0.443825473, 3.93195214)
( 0.447940201, 3.97627537)
( 0.452093076, 4.02126135)
( 0.456284453, 4.06692503)
( 0.460514689, 4.11328189)
( 0.464784143, 4.1603479)
( 0.469093179, 4.20813957)
( 0.473442165, 4.25667398)
( 0.477831471, 4.3059688)
( 0.482261469, 4.3560423)
( 0.486732539, 4.40691342)
( 0.49124506, 4.45860175)
( 0.495799417, 4.5111276)
( 0.500395998, 4.564512)
( 0.505035194, 4.61877679)
( 0.5097174, 4.6739446)
( 0.514443015, 4.73003893)
( 0.519212441, 4.78708417)
( 0.524026085, 4.84510567)
( 0.528884356, 4.90412976)
( 0.533787669, 4.96418383)
( 0.538736441, 5.02529638)
( 0.543731093, 5.08749708)
( 0.54877205, 5.15081681)
( 0.553859743, 5.21528779)
( 0.558994603, 5.28094359)
( 0.56417707, 5.34781925)
( 0.569407583, 5.41595134)
( 0.574686589, 5.48537811)
( 0.580014536, 5.5561395)
( 0.585391879, 5.62827733)
( 0.590819076, 5.70183539)
( 0.596296588, 5.77685955)
( 0.601824883, 5.85339792)
( 0.607404431, 5.931501)
( 0.613035707, 6.01122184)
( 0.618719191, 6.09261621)
( 0.624455367, 6.17574283)
( 0.630244724, 6.26066353)
( 0.636087753, 6.34744354)
( 0.641984954, 6.4361517)
( 0.647936828, 6.52686078)
( 0.653943882, 6.61964778)
( 0.660006628, 6.71459427)
( 0.666125581, 6.81178678)
( 0.672301264, 6.91131723)
( 0.678534202, 7.01328339)
( 0.684824926, 7.11778943)
( 0.691173971, 7.22494647)
( 0.697581879, 7.33487331)
( 0.704049195, 7.44769712)
( 0.710576469, 7.56355429)
( 0.717164258, 7.68259143)
( 0.723813123, 7.80496638)
( 0.73052363, 7.93084953)
( 0.73729635, 8.06042518)
( 0.744131861, 8.19389318)
( 0.751030744, 8.33147084)
( 0.757993587, 8.47339508)
( 0.765020982, 8.61992499)
( 0.772113529, 8.77134478)
( 0.779271831, 8.92796734)
( 0.786496499, 9.09013835)
( 0.793788146, 9.25824125)
( 0.801147395, 9.43270319)
( 0.808574872, 9.6140022)
( 0.816071209, 9.80267597)
( 0.823637045, 9.99933256)
( 0.831273024, 10.2046638)
( 0.838979797, 10.419462)
( 0.84675802, 10.6446409)
( 0.854608355, 10.8812633)
( 0.862531471, 11.1305756)
( 0.870528042, 11.3940549)
( 0.87859875, 11.6734709)
( 0.886744282, 11.9709715)
( 0.894965332, 12.2892013)
( 0.903262599, 12.6314722)
( 0.911636791, 13.0020139)
( 0.92008862, 13.4063562)
( 0.928618807, 13.8519343)
( 0.937228077, 14.349097)
( 0.945917165, 14.9128895)
( 0.954686809, 15.5664601)
( 0.963537757, 16.3482755)
( 0.972470763, 17.3297931)
( 0.981486587, 18.6696114)
( 0.990585997, 20.8643926)
( 0.999769768, 32.2009507)
};
\addplot [blue, dashed]
coordinates {
( 0.01, 3.66804948)
( 0.0100821039, 3.66804948)
( 0.010164882, 3.66804948)
( 0.0102483397, 3.66804948)
( 0.0103324826, 3.66804948)
( 0.0104173163, 3.66804948)
( 0.0105028466, 3.66804948)
( 0.0105890791, 3.66804948)
( 0.0106760196, 3.66804948)
( 0.0107636739, 3.66804948)
( 0.0108520479, 3.66804948)
( 0.0109411475, 3.66804948)
( 0.0110309787, 3.66804948)
( 0.0111215473, 3.66804948)
( 0.0112128596, 3.66804948)
( 0.0113049216, 3.66804948)
( 0.0113977395, 3.66804948)
( 0.0114913194, 3.66804948)
( 0.0115856677, 3.66804948)
( 0.0116807906, 3.66804948)
( 0.0117766945, 3.66804948)
( 0.0118733858, 3.66804948)
( 0.0119708709, 3.66804948)
( 0.0120691565, 3.66804948)
( 0.012168249, 3.66804948)
( 0.0122681551, 3.66804948)
( 0.0123688815, 3.66804948)
( 0.0124704349, 3.66804948)
( 0.0125728221, 3.66804948)
( 0.0126760499, 3.66804948)
( 0.0127801253, 3.66804948)
( 0.0128850552, 3.66804948)
( 0.0129908465, 3.66804948)
( 0.0130975065, 3.66804948)
( 0.0132050422, 3.66804948)
( 0.0133134608, 3.66804948)
( 0.0134227695, 3.66804948)
( 0.0135329758, 3.66804948)
( 0.0136440868, 3.66804948)
( 0.0137561102, 3.66804948)
( 0.0138690532, 3.66804948)
( 0.0139829236, 3.66804948)
( 0.0140977289, 3.66804948)
( 0.0142134769, 3.66804948)
( 0.0143301751, 3.66804948)
( 0.0144478315, 3.66804948)
( 0.0145664539, 3.66804948)
( 0.0146860502, 3.66804948)
( 0.0148066284, 3.66804948)
( 0.0149281967, 3.66804948)
( 0.0150507631, 3.66804948)
( 0.0151743358, 3.66804948)
( 0.015298923, 3.66804948)
( 0.0154245332, 3.66804948)
( 0.0155511747, 3.66804948)
( 0.015678856, 3.66804948)
( 0.0158075856, 3.66804948)
( 0.0159373721, 3.66804948)
( 0.0160682242, 3.66804948)
( 0.0162001506, 3.66804948)
( 0.0163331603, 3.66804948)
( 0.0164672619, 3.66804948)
( 0.0166024646, 3.66804948)
( 0.0167387774, 3.66804948)
( 0.0168762094, 3.66804948)
( 0.0170147697, 3.66804948)
( 0.0171544677, 3.66804948)
( 0.0172953126, 3.66804948)
( 0.0174373139, 3.66804948)
( 0.0175804811, 3.66804948)
( 0.0177248238, 3.66804948)
( 0.0178703516, 3.66804948)
( 0.0180170742, 3.66804948)
( 0.0181650015, 3.66804948)
( 0.0183141433, 3.66804948)
( 0.0184645097, 3.66804948)
( 0.0186161105, 3.66804948)
( 0.0187689561, 3.66804948)
( 0.0189230567, 3.66804948)
( 0.0190784224, 3.66804948)
( 0.0192350638, 3.66804948)
( 0.0193929912, 3.66804948)
( 0.0195522153, 3.66804948)
( 0.0197127467, 3.66804948)
( 0.0198745961, 3.66804948)
( 0.0200377744, 3.66804948)
( 0.0202022924, 3.66804948)
( 0.0203681612, 3.66804948)
( 0.0205353918, 3.66804948)
( 0.0207039955, 3.66804948)
( 0.0208739834, 3.66804948)
( 0.0210453671, 3.66804948)
( 0.0212181578, 3.66804948)
( 0.0213923673, 3.66804948)
( 0.021568007, 3.66804948)
( 0.0217450889, 3.66804948)
( 0.0219236246, 3.66804948)
( 0.0221036262, 3.66804948)
( 0.0222851057, 3.66804948)
( 0.0224680752, 3.66804948)
( 0.0226525469, 3.66804948)
( 0.0228385332, 3.66804948)
( 0.0230260466, 3.66804948)
( 0.0232150995, 3.66804949)
( 0.0234057046, 3.66804949)
( 0.0235978747, 3.66804949)
( 0.0237916225, 3.66804949)
( 0.0239869611, 3.66804949)
( 0.0241839035, 3.6680495)
( 0.0243824629, 3.6680495)
( 0.0245826525, 3.6680495)
( 0.0247844858, 3.66804951)
( 0.0249879762, 3.66804951)
( 0.0251931373, 3.66804952)
( 0.0253999829, 3.66804953)
( 0.0256085267, 3.66804954)
( 0.0258187828, 3.66804955)
( 0.0260307652, 3.66804956)
( 0.0262444881, 3.66804957)
( 0.0264599656, 3.66804958)
( 0.0266772124, 3.6680496)
( 0.0268962428, 3.66804962)
( 0.0271170715, 3.66804964)
( 0.0273397134, 3.66804967)
( 0.0275641832, 3.66804969)
( 0.027790496, 3.66804973)
( 0.0280186669, 3.66804976)
( 0.0282487112, 3.6680498)
( 0.0284806443, 3.66804985)
( 0.0287144816, 3.6680499)
( 0.0289502388, 3.66804996)
( 0.0291879316, 3.66805003)
( 0.0294275761, 3.6680501)
( 0.029669188, 3.66805019)
( 0.0299127838, 3.66805028)
( 0.0301583795, 3.66805039)
( 0.0304059917, 3.66805051)
( 0.0306556369, 3.66805065)
( 0.0309073317, 3.6680508)
( 0.0311610931, 3.66805097)
( 0.0314169379, 3.66805116)
( 0.0316748834, 3.66805137)
( 0.0319349466, 3.66805161)
( 0.0321971451, 3.66805187)
( 0.0324614964, 3.66805217)
( 0.032728018, 3.6680525)
( 0.032996728, 3.66805286)
( 0.0332676441, 3.66805327)
( 0.0335407846, 3.66805372)
( 0.0338161676, 3.66805422)
( 0.0340938117, 3.66805477)
( 0.0343737353, 3.66805538)
( 0.0346559572, 3.66805606)
( 0.0349404963, 3.66805681)
( 0.0352273715, 3.66805764)
( 0.0355166021, 3.66805855)
( 0.0358082074, 3.66805956)
( 0.0361022069, 3.66806066)
( 0.0363986202, 3.66806188)
( 0.0366974672, 3.66806322)
( 0.0369987679, 3.6680647)
( 0.0373025423, 3.66806631)
( 0.0376088109, 3.66806809)
( 0.0379175941, 3.66807003)
( 0.0382289124, 3.66807216)
( 0.0385427869, 3.66807448)
( 0.0388592383, 3.66807703)
( 0.039178288, 3.6680798)
( 0.0394999572, 3.66808284)
( 0.0398242674, 3.66808615)
( 0.0401512403, 3.66808975)
( 0.0404808978, 3.66809367)
( 0.0408132619, 3.66809795)
( 0.0411483549, 3.66810259)
( 0.0414861991, 3.66810763)
( 0.0418268171, 3.66811311)
( 0.0421702318, 3.66811905)
( 0.042516466, 3.66812549)
( 0.0428655429, 3.66813247)
( 0.0432174859, 3.66814003)
( 0.0435723185, 3.6681482)
( 0.0439300644, 3.66815703)
( 0.0442907475, 3.66816657)
( 0.044654392, 3.66817687)
( 0.0450210221, 3.66818799)
( 0.0453906625, 3.66819996)
( 0.0457633377, 3.66821287)
( 0.0461390727, 3.66822676)
( 0.0465178927, 3.6682417)
( 0.0468998229, 3.66825777)
( 0.0472848889, 3.66827503)
( 0.0476731165, 3.66829356)
( 0.0480645316, 3.66831345)
( 0.0484591603, 3.66833478)
( 0.0488570291, 3.66835763)
( 0.0492581645, 3.66838211)
( 0.0496625935, 3.6684083)
( 0.0500703429, 3.66843632)
( 0.0504814402, 3.66846628)
( 0.0508959127, 3.66849828)
( 0.0513137882, 3.66853245)
( 0.0517350946, 3.66856891)
( 0.0521598601, 3.66860779)
( 0.0525881131, 3.66864923)
( 0.0530198822, 3.66869337)
( 0.0534551963, 3.66874036)
( 0.0538940845, 3.66879035)
( 0.0543365762, 3.66884351)
( 0.0547827009, 3.66890001)
( 0.0552324885, 3.66896001)
( 0.0556859689, 3.66902371)
( 0.0561431727, 3.66909129)
( 0.0566041303, 3.66916296)
( 0.0570688725, 3.66923891)
( 0.0575374304, 3.66931936)
( 0.0580098353, 3.66940454)
( 0.0584861189, 3.66949466)
( 0.058966313, 3.66958997)
( 0.0594504497, 3.66969072)
( 0.0599385613, 3.66979716)
( 0.0604306805, 3.66990955)
( 0.0609268402, 3.67002816)
( 0.0614270735, 3.67015329)
( 0.061931414, 3.67028522)
( 0.0624398953, 3.67042425)
( 0.0629525515, 3.67057069)
( 0.0634694167, 3.67072487)
( 0.0639905256, 3.6708871)
( 0.064515913, 3.67105775)
( 0.0650456141, 3.67123714)
( 0.0655796642, 3.67142565)
( 0.0661180991, 3.67162365)
( 0.0666609547, 3.67183152)
( 0.0672082674, 3.67204964)
( 0.0677600738, 3.67227843)
( 0.0683164107, 3.67251829)
( 0.0688773153, 3.67276966)
( 0.0694428252, 3.67303296)
( 0.0700129781, 3.67330865)
( 0.0705878123, 3.67359718)
( 0.071167366, 3.67389901)
( 0.0717516781, 3.67421464)
( 0.0723407877, 3.67454454)
( 0.072934734, 3.67488923)
( 0.0735335569, 3.67524921)
( 0.0741372964, 3.67562501)
( 0.0747459928, 3.67601716)
( 0.0753596869, 3.67642622)
( 0.0759784196, 3.67685274)
( 0.0766022323, 3.67729729)
( 0.0772311668, 3.67776045)
( 0.0778652651, 3.67824281)
( 0.0785045696, 3.67874498)
( 0.0791491231, 3.67926757)
( 0.0797989685, 3.6798112)
( 0.0804541495, 3.68037652)
( 0.0811147098, 3.68096416)
( 0.0817806935, 3.68157478)
( 0.0824521452, 3.68220906)
( 0.0831291098, 3.68286767)
( 0.0838116325, 3.6835513)
( 0.084499759, 3.68426065)
( 0.0851935353, 3.68499644)
( 0.0858930078, 3.68575937)
( 0.0865982233, 3.68655018)
( 0.0873092288, 3.68736962)
( 0.0880260719, 3.68821843)
( 0.0887488007, 3.68909737)
( 0.0894774633, 3.69000721)
( 0.0902121085, 3.69094872)
( 0.0909527855, 3.6919227)
( 0.0916995436, 3.69292994)
( 0.092452433, 3.69397125)
( 0.0932115039, 3.69504744)
( 0.0939768071, 3.69615933)
( 0.0947483937, 3.69730776)
( 0.0955263153, 3.69849356)
( 0.096310624, 3.69971757)
( 0.0971013722, 3.70098066)
( 0.0978986127, 3.70228368)
( 0.0987023989, 3.7036275)
( 0.0995127844, 3.705013)
( 0.100329824, 3.70644107)
( 0.101153571, 3.70791258)
( 0.101984082, 3.70942845)
( 0.102821411, 3.71098956)
( 0.103665615, 3.71259683)
( 0.104516751, 3.71425118)
( 0.105374875, 3.71595351)
( 0.106240044, 3.71770477)
( 0.107112316, 3.71950588)
( 0.107991751, 3.72135777)
( 0.108878406, 3.72326139)
( 0.10977234, 3.72521768)
( 0.110673614, 3.7272276)
( 0.111582288, 3.72929209)
( 0.112498423, 3.73141211)
( 0.113422079, 3.73358863)
( 0.114353319, 3.73582262)
( 0.115292205, 3.73811504)
( 0.116238799, 3.74046686)
( 0.117193166, 3.74287907)
( 0.118155368, 3.74535264)
( 0.11912547, 3.74788854)
( 0.120103537, 3.75048778)
( 0.121089634, 3.75315133)
( 0.122083828, 3.75588018)
( 0.123086184, 3.75867532)
( 0.12409677, 3.76153775)
( 0.125115654, 3.76446846)
( 0.126142902, 3.76746845)
( 0.127178585, 3.77053872)
( 0.128222772, 3.77368026)
( 0.129275531, 3.77689408)
( 0.130336934, 3.78018118)
( 0.131407052, 3.78354257)
( 0.132485955, 3.78697924)
( 0.133573717, 3.7904922)
( 0.13467041, 3.79408246)
( 0.135776107, 3.79775102)
( 0.136890882, 3.80149889)
( 0.138014811, 3.80532708)
( 0.139147967, 3.80923659)
( 0.140290426, 3.81322844)
( 0.141442266, 3.81730363)
( 0.142603563, 3.82146316)
( 0.143774394, 3.82570805)
( 0.144954838, 3.8300393)
( 0.146144975, 3.83445793)
( 0.147344882, 3.83896494)
( 0.148554642, 3.84356133)
( 0.149774334, 3.84824812)
( 0.15100404, 3.85302631)
( 0.152243843, 3.85789692)
( 0.153493825, 3.86286094)
( 0.15475407, 3.86791938)
( 0.156024662, 3.87307325)
( 0.157305686, 3.87832356)
( 0.158597227, 3.88367131)
( 0.159899373, 3.88911751)
( 0.16121221, 3.89466316)
( 0.162535825, 3.90030927)
( 0.163870309, 3.90605684)
( 0.165215748, 3.91190687)
( 0.166572235, 3.91786038)
( 0.167939858, 3.92391837)
( 0.169318711, 3.93008183)
( 0.170708884, 3.93635178)
( 0.172110471, 3.94272922)
( 0.173523566, 3.94921516)
( 0.174948263, 3.95581058)
( 0.176384657, 3.96251652)
( 0.177832845, 3.96933396)
( 0.179292922, 3.97626391)
( 0.180764988, 3.98330737)
( 0.18224914, 3.99046536)
( 0.183745477, 3.99773888)
( 0.1852541, 4.00512894)
( 0.186775109, 4.01263654)
( 0.188308606, 4.02026269)
( 0.189854694, 4.02800841)
( 0.191413476, 4.03587469)
( 0.192985056, 4.04386256)
( 0.194569539, 4.05197303)
( 0.196167032, 4.0602071)
( 0.19777764, 4.0685658)
( 0.199401472, 4.07705014)
( 0.201038637, 4.08566113)
( 0.202689243, 4.0943998)
( 0.204353402, 4.10326717)
( 0.206031224, 4.11226427)
( 0.207722821, 4.12139211)
( 0.209428308, 4.13065172)
( 0.211147797, 4.14004414)
( 0.212881403, 4.14957039)
( 0.214629243, 4.15923151)
( 0.216391434, 4.16902854)
( 0.218168093, 4.17896252)
( 0.219959339, 4.18903448)
( 0.221765292, 4.19924548)
( 0.223586072, 4.20959657)
( 0.225421802, 4.22008878)
( 0.227272604, 4.23072319)
( 0.229138601, 4.24150085)
( 0.231019919, 4.25242282)
( 0.232916684, 4.26349016)
( 0.234829022, 4.27470395)
( 0.23675706, 4.28606527)
( 0.238700929, 4.29757518)
( 0.240660758, 4.30923477)
( 0.242636677, 4.32104514)
( 0.24462882, 4.33300737)
( 0.246637319, 4.34512255)
( 0.248662309, 4.35739179)
( 0.250703924, 4.3698162)
( 0.252762302, 4.38239688)
( 0.25483758, 4.39513496)
( 0.256929897, 4.40803156)
( 0.259039393, 4.4210878)
( 0.261166208, 4.43430481)
( 0.263310486, 4.44768375)
( 0.265472368, 4.46122574)
( 0.267652001, 4.47493195)
( 0.26984953, 4.48880354)
( 0.2720651, 4.50284166)
( 0.274298862, 4.51704749)
( 0.276550964, 4.5314222)
( 0.278821556, 4.54596699)
( 0.281110791, 4.56068304)
( 0.283418821, 4.57557155)
( 0.285745801, 4.59063374)
( 0.288091887, 4.6058708)
( 0.290457235, 4.62128397)
( 0.292842003, 4.63687448)
( 0.295246351, 4.65264355)
( 0.29767044, 4.66859245)
( 0.300114432, 4.68472241)
( 0.30257849, 4.70103471)
( 0.305062778, 4.71753061)
( 0.307567464, 4.73421139)
( 0.310092714, 4.75107834)
( 0.312638697, 4.76813276)
( 0.315205584, 4.78537596)
( 0.317793546, 4.80280924)
( 0.320402756, 4.82043394)
( 0.323033389, 4.83825138)
( 0.32568562, 4.85626292)
( 0.328359628, 4.8744699)
( 0.331055589, 4.8928737)
( 0.333773686, 4.91147567)
( 0.3365141, 4.93027722)
( 0.339277013, 4.94927973)
( 0.342062611, 4.9684846)
( 0.34487108, 4.98789326)
( 0.347702607, 5.00750713)
( 0.350557383, 5.02732765)
( 0.353435597, 5.04735627)
( 0.356337442, 5.06759444)
( 0.359263113, 5.08804365)
( 0.362212805, 5.10870536)
( 0.365186714, 5.12958109)
( 0.368185041, 5.15067233)
( 0.371207985, 5.1719806)
( 0.374255749, 5.19350744)
( 0.377328536, 5.21525439)
( 0.380426552, 5.23722301)
( 0.383550004, 5.25941485)
( 0.386699101, 5.28183151)
( 0.389874053, 5.30447458)
( 0.393075072, 5.32734567)
( 0.396302373, 5.3504464)
( 0.399556172, 5.37377839)
( 0.402836686, 5.39734331)
( 0.406144133, 5.4211428)
( 0.409478737, 5.44517855)
( 0.412840719, 5.46945225)
( 0.416230303, 5.49396559)
( 0.419647718, 5.51872029)
( 0.423093191, 5.54371809)
( 0.426566953, 5.56896074)
( 0.430069236, 5.59444998)
( 0.433600274, 5.62018761)
( 0.437160303, 5.64617541)
( 0.440749561, 5.67241518)
( 0.444368288, 5.69890875)
( 0.448016727, 5.72565796)
( 0.451695121, 5.75266465)
( 0.455403716, 5.7799307)
( 0.45914276, 5.80745799)
( 0.462912503, 5.83524842)
( 0.466713197, 5.8633039)
( 0.470545096, 5.89162638)
( 0.474408456, 5.9202178)
( 0.478303537, 5.94908012)
( 0.482230597, 5.97821533)
( 0.4861899, 6.00762543)
( 0.490181711, 6.03731244)
( 0.494206296, 6.06727839)
( 0.498263924, 6.09752533)
( 0.502354867, 6.12805534)
( 0.506479399, 6.1588705)
( 0.510637794, 6.18997292)
( 0.514830331, 6.22136472)
( 0.519057291, 6.25304804)
( 0.523318956, 6.28502505)
( 0.527615611, 6.31729793)
( 0.531947543, 6.34986887)
( 0.536315042, 6.38274009)
( 0.540718399, 6.41591382)
( 0.545157911, 6.44939233)
( 0.549633872, 6.48317789)
( 0.554146582, 6.51727279)
( 0.558696344, 6.55167935)
( 0.563283461, 6.58639991)
( 0.56790824, 6.62143681)
( 0.572570991, 6.65679244)
( 0.577272024, 6.69246919)
( 0.582011655, 6.72846948)
( 0.5867902, 6.76479574)
( 0.591607978, 6.80145044)
};
\addplot [blue, dashed]
coordinates {
( 0.01, 4.48502226e-20)
( 0.0100821039, 6.51514489e-20)
( 0.010164882, 9.4354584e-20)
( 0.0102483397, 1.36236078e-19)
( 0.0103324826, 1.96120111e-19)
( 0.0104173163, 2.81490392e-19)
( 0.0105028466, 4.02834785e-19)
( 0.0105890791, 5.74807868e-19)
( 0.0106760196, 8.17826383e-19)
( 0.0107636739, 1.16025231e-18)
( 0.0108520479, 1.6413713e-18)
( 0.0109411475, 2.31544446e-18)
( 0.0110309787, 3.25720456e-18)
( 0.0111215473, 4.5692902e-18)
( 0.0112128596, 6.39227308e-18)
( 0.0113049216, 8.91814475e-18)
( 0.0113977395, 1.24084062e-17)
( 0.0114913194, 1.72182643e-17)
( 0.0115856677, 2.38289073e-17)
( 0.0116807906, 3.28904423e-17)
( 0.0117766945, 4.52788601e-17)
( 0.0118733858, 6.21714111e-17)
( 0.0119708709, 8.51460761e-17)
( 0.0120691565, 1.16312491e-16)
( 0.012168249, 1.58483824e-16)
( 0.0122681551, 2.15401821e-16)
( 0.0123688815, 2.92030731e-16)
( 0.0124704349, 3.94940195e-16)
( 0.0125728221, 5.32802774e-16)
( 0.0126760499, 7.17038827e-16)
( 0.0127801253, 9.62650291e-16)
( 0.0128850552, 1.28929605e-15)
( 0.0129908465, 1.72267548e-15)
( 0.0130975065, 2.29630421e-15)
( 0.0132050422, 3.05378775e-15)
( 0.0133134608, 4.05172563e-15)
( 0.0134227695, 5.36341217e-15)
( 0.0135329758, 7.08354123e-15)
( 0.0136440868, 9.33417341e-15)
( 0.0137561102, 1.2272287e-14)
( 0.0138690532, 1.60993107e-14)
( 0.0139829236, 2.10731321e-14)
( 0.0140977289, 2.75231882e-14)
( 0.0142134769, 3.58693896e-14)
( 0.0143301751, 4.66457975e-14)
( 0.0144478315, 6.05301813e-14)
( 0.0145664539, 7.83808392e-14)
( 0.0146860502, 1.01282364e-13)
( 0.0148066284, 1.30602407e-13)
( 0.0149281967, 1.68061929e-13)
( 0.0150507631, 2.15821966e-13)
( 0.0151743358, 2.76590553e-13)
( 0.015298923, 3.5375423e-13)
( 0.0154245332, 4.51539438e-13)
( 0.0155511747, 5.75210187e-13)
( 0.015678856, 7.31309664e-13)
( 0.0158075856, 9.27954948e-13)
( 0.0159373721, 1.17519578e-12)
( 0.0160682242, 1.48545042e-12)
( 0.0162001506, 1.8740342e-12)
( 0.0163331603, 2.35979906e-12)
( 0.0164672619, 2.96590603e-12)
( 0.0166024646, 3.72075644e-12)
( 0.0167387774, 4.65911223e-12)
( 0.0168762094, 5.82344137e-12)
( 0.0170147697, 7.26553042e-12)
( 0.0171544677, 9.04841375e-12)
( 0.0172953126, 1.12486773e-11)
( 0.0174373139, 1.39592042e-11)
( 0.0175804811, 1.72924423e-11)
( 0.0177248238, 2.13842832e-11)
( 0.0178703516, 2.63986617e-11)
( 0.0180170742, 3.25329988e-11)
( 0.0181650015, 4.00246295e-11)
( 0.0183141433, 4.91583843e-11)
( 0.0184645097, 6.02755115e-11)
( 0.0186161105, 7.37841627e-11)
( 0.0187689561, 9.01716919e-11)
( 0.0189230567, 1.10019059e-10)
( 0.0190784224, 1.34017666e-10)
( 0.0192350638, 1.62989009e-10)
( 0.0193929912, 1.97907577e-10)
( 0.0195522153, 2.39927478e-10)
( 0.0197127467, 2.90413375e-10)
( 0.0198745961, 3.50976342e-10)
( 0.0200377744, 4.23515368e-10)
( 0.0202022924, 5.10265334e-10)
( 0.0203681612, 6.13852351e-10)
( 0.0205353918, 7.37357528e-10)
( 0.0207039955, 8.84390305e-10)
( 0.0208739834, 1.05917267e-9)
( 0.0210453671, 1.26663573e-9)
( 0.0212181578, 1.51253027e-9)
( 0.0213923673, 1.80355311e-9)
( 0.021568007, 2.14749138e-9)
( 0.0217450889, 2.55338687e-9)
( 0.0219236246, 3.03172316e-9)
( 0.0221036262, 3.59463811e-9)
( 0.0222851057, 4.25616509e-9)
( 0.0224680752, 5.03250621e-9)
( 0.0226525469, 5.94234146e-9)
( 0.0228385332, 7.00717787e-9)
( 0.0230260466, 8.25174352e-9)
( 0.0232150995, 9.70443127e-9)
( 0.0234057046, 1.13977979e-8)
( 0.0235978747, 1.3369125e-8)
( 0.0237916225, 1.56610478e-8)
( 0.0239869611, 1.832226e-8)
( 0.0241839035, 2.14083018e-8)
( 0.0243824629, 2.49824407e-8)
( 0.0245826525, 2.91166542e-8)
( 0.0247844858, 3.38927238e-8)
( 0.0249879762, 3.94034537e-8)
( 0.0251931373, 4.57540236e-8)
( 0.0253999829, 5.30634912e-8)
( 0.0256085267, 6.14664565e-8)
( 0.0258187828, 7.11149047e-8)
( 0.0260307652, 8.21802427e-8)
( 0.0262444881, 9.48555481e-8)
( 0.0264599656, 1.09358049e-7)
( 0.0266772124, 1.25931853e-7)
( 0.0268962428, 1.44850955e-7)
( 0.0271170715, 1.66422529e-7)
( 0.0273397134, 1.90990557e-7)
( 0.0275641832, 2.18939787e-7)
( 0.027790496, 2.5070008e-7)
( 0.0280186669, 2.86751153e-7)
( 0.0282487112, 3.27627759e-7)
( 0.0284806443, 3.73925343e-7)
( 0.0287144816, 4.26306188e-7)
( 0.0289502388, 4.8550612e-7)
( 0.0291879316, 5.52341774e-7)
( 0.0294275761, 6.277185e-7)
( 0.029669188, 7.12638919e-7)
( 0.0299127838, 8.08212197e-7)
( 0.0301583795, 9.15664071e-7)
( 0.0304059917, 1.03634768e-6)
( 0.0306556369, 1.17175528e-6)
( 0.0309073317, 1.3235308e-6)
( 0.0311610931, 1.49348347e-6)
( 0.0314169379, 1.68360236e-6)
( 0.0316748834, 1.89607213e-6)
( 0.0319349466, 2.13328979e-6)
( 0.0321971451, 2.39788278e-6)
( 0.0324614964, 2.6927283e-6)
( 0.032728018, 3.02097395e-6)
( 0.032996728, 3.3860598e-6)
( 0.0332676441, 3.791742e-6)
( 0.0335407846, 4.2421179e-6)
( 0.0338161676, 4.74165277e-6)
( 0.0340938117, 5.29520833e-6)
( 0.0343737353, 5.90807302e-6)
( 0.0346559572, 6.58599408e-6)
( 0.0349404963, 7.33521169e-6)
( 0.0352273715, 8.16249505e-6)
( 0.0355166021, 9.07518062e-6)
( 0.0358082074, 1.00812125e-5)
( 0.0361022069, 1.11891852e-5)
( 0.0363986202, 1.24083885e-5)
( 0.0366974672, 1.37488552e-5)
( 0.0369987679, 1.52214107e-5)
( 0.0373025423, 1.68377261e-5)
( 0.0376088109, 1.8610373e-5)
( 0.0379175941, 2.05528818e-5)
( 0.0382289124, 2.26798023e-5)
( 0.0385427869, 2.50067677e-5)
( 0.0388592383, 2.75505611e-5)
( 0.039178288, 3.03291853e-5)
( 0.0394999572, 3.33619358e-5)
( 0.0398242674, 3.66694766e-5)
( 0.0401512403, 4.02739194e-5)
( 0.0404808978, 4.41989067e-5)
( 0.0408132619, 4.84696968e-5)
( 0.0411483549, 5.31132538e-5)
( 0.0414861991, 5.81583398e-5)
( 0.0418268171, 6.36356113e-5)
( 0.0421702318, 6.95777185e-5)
( 0.042516466, 7.60194089e-5)
( 0.0428655429, 8.29976333e-5)
( 0.0432174859, 9.05516565e-5)
( 0.0435723185, 9.87231707e-5)
( 0.0439300644, 0.000107556413)
( 0.0442907475, 0.000117098286)
( 0.044654392, 0.000127398481)
( 0.0450210221, 0.00013850961)
( 0.0453906625, 0.00015048733)
( 0.0457633377, 0.000163390484)
( 0.0461390727, 0.000177281235)
( 0.0465178927, 0.000192225208)
( 0.0468998229, 0.000208291638)
( 0.0472848889, 0.00022555351)
( 0.0476731165, 0.000244087718)
( 0.0480645316, 0.000263975214)
( 0.0484591603, 0.000285301163)
( 0.0488570291, 0.000308155106)
( 0.0492581645, 0.000332631121)
( 0.0496625935, 0.000358827984)
( 0.0500703429, 0.000386849339)
( 0.0504814402, 0.000416803866)
( 0.0508959127, 0.000448805448)
( 0.0513137882, 0.000482973349)
( 0.0517350946, 0.000519432385)
( 0.0521598601, 0.0005583131)
( 0.0525881131, 0.000599751944)
( 0.0530198822, 0.000643891446)
( 0.0534551963, 0.0006908804)
( 0.0538940845, 0.000740874039)
( 0.0543365762, 0.000794034218)
( 0.0547827009, 0.000850529589)
( 0.0552324885, 0.000910535786)
( 0.0556859689, 0.000974235602)
( 0.0561431727, 0.00104181917)
( 0.0566041303, 0.00111348413)
( 0.0570688725, 0.00118943582)
( 0.0575374304, 0.00126988746)
( 0.0580098353, 0.00135506029)
( 0.0584861189, 0.00144518376)
( 0.058966313, 0.00154049574)
( 0.0594504497, 0.00164124261)
( 0.0599385613, 0.00174767948)
( 0.0604306805, 0.00186007035)
( 0.0609268402, 0.00197868824)
( 0.0614270735, 0.00210381536)
( 0.061931414, 0.00223574326)
( 0.0624398953, 0.00237477299)
( 0.0629525515, 0.00252121521)
( 0.0634694167, 0.00267539037)
( 0.0639905256, 0.00283762881)
( 0.064515913, 0.0030082709)
( 0.0650456141, 0.00318766716)
( 0.0655796642, 0.00337617838)
( 0.0661180991, 0.00357417574)
( 0.0666609547, 0.0037820409)
( 0.0672082674, 0.0040001661)
( 0.0677600738, 0.00422895427)
( 0.0683164107, 0.0044688191)
( 0.0688773153, 0.00472018513)
( 0.0694428252, 0.00498348781)
( 0.0700129781, 0.00525917358)
( 0.0705878123, 0.00554769991)
( 0.071167366, 0.00584953539)
( 0.0717516781, 0.00616515972)
( 0.0723407877, 0.00649506379)
( 0.072934734, 0.00683974969)
( 0.0735335569, 0.00719973071)
( 0.0741372964, 0.00757553142)
( 0.0747459928, 0.00796768759)
( 0.0753596869, 0.00837674626)
( 0.0759784196, 0.00880326567)
( 0.0766022323, 0.0092478153)
( 0.0772311668, 0.00971097579)
( 0.0778652651, 0.0101933389)
( 0.0785045696, 0.0106955077)
( 0.0791491231, 0.0112180959)
( 0.0797989685, 0.0117617286)
( 0.0804541495, 0.0123270418)
( 0.0811147098, 0.0129146821)
( 0.0817806935, 0.0135253071)
( 0.0824521452, 0.0141595851)
( 0.0831291098, 0.0148181949)
( 0.0838116325, 0.0155018258)
( 0.084499759, 0.0162111777)
( 0.0851935353, 0.0169469604)
( 0.0858930078, 0.0177098942)
( 0.0865982233, 0.0185007093)
( 0.0873092288, 0.0193201458)
( 0.0880260719, 0.0201689535)
( 0.0887488007, 0.0210478919)
( 0.0894774633, 0.0219577299)
( 0.0902121085, 0.0228992457)
( 0.0909527855, 0.0238732266)
( 0.0916995436, 0.024880469)
( 0.092452433, 0.025921778)
( 0.0932115039, 0.0269979674)
( 0.0939768071, 0.0281098594)
( 0.0947483937, 0.0292582843)
( 0.0955263153, 0.0304440809)
( 0.096310624, 0.0316680954)
( 0.0971013722, 0.0329311821)
( 0.0978986127, 0.0342342026)
( 0.0987023989, 0.0355780259)
( 0.0995127844, 0.0369635279)
( 0.100329824, 0.0383915918)
( 0.101153571, 0.039863107)
( 0.101984082, 0.0413789699)
( 0.102821411, 0.042940083)
( 0.103665615, 0.0445473547)
( 0.104516751, 0.0462016995)
( 0.105374875, 0.0479040377)
( 0.106240044, 0.0496552948)
( 0.107112316, 0.0514564018)
( 0.107991751, 0.0533082947)
( 0.108878406, 0.0552119142)
( 0.10977234, 0.0571682061)
( 0.110673614, 0.0591781202)
( 0.111582288, 0.0612426108)
( 0.112498423, 0.0633626365)
( 0.113422079, 0.0655391593)
( 0.114353319, 0.0677731454)
( 0.115292205, 0.0700655641)
( 0.116238799, 0.0724173882)
( 0.117193166, 0.0748295938)
( 0.118155368, 0.0773031597)
( 0.11912547, 0.0798390677)
( 0.120103537, 0.0824383021)
( 0.121089634, 0.0851018498)
( 0.122083828, 0.0878306997)
( 0.123086184, 0.0906258431)
( 0.12409677, 0.0934882732)
( 0.125115654, 0.0964189851)
( 0.126142902, 0.0994189756)
( 0.127178585, 0.102489243)
( 0.128222772, 0.105630786)
( 0.129275531, 0.108844607)
( 0.130336934, 0.112131708)
( 0.131407052, 0.115493091)
( 0.132485955, 0.118929761)
( 0.133573717, 0.122442723)
( 0.13467041, 0.126032981)
( 0.135776107, 0.129701543)
( 0.136890882, 0.133449416)
( 0.138014811, 0.137277605)
( 0.139147967, 0.141187118)
( 0.140290426, 0.145178964)
( 0.141442266, 0.14925415)
( 0.142603563, 0.153413684)
( 0.143774394, 0.157658575)
( 0.144954838, 0.161989829)
( 0.146144975, 0.166408456)
( 0.147344882, 0.170915462)
( 0.148554642, 0.175511857)
( 0.149774334, 0.180198647)
( 0.15100404, 0.184976839)
( 0.152243843, 0.189847442)
( 0.153493825, 0.194811461)
( 0.15475407, 0.199869903)
( 0.156024662, 0.205023776)
( 0.157305686, 0.210274084)
( 0.158597227, 0.215621834)
( 0.159899373, 0.221068032)
( 0.16121221, 0.226613682)
( 0.162535825, 0.23225979)
( 0.163870309, 0.23800736)
( 0.165215748, 0.243857398)
( 0.166572235, 0.249810907)
( 0.167939858, 0.255868892)
( 0.169318711, 0.262032358)
( 0.170708884, 0.268302308)
( 0.172110471, 0.274679747)
( 0.173523566, 0.28116568)
( 0.174948263, 0.287761109)
( 0.176384657, 0.294467041)
( 0.177832845, 0.30128448)
( 0.179292922, 0.30821443)
( 0.180764988, 0.315257898)
( 0.18224914, 0.322415888)
( 0.183745477, 0.329689408)
( 0.1852541, 0.337079465)
( 0.186775109, 0.344587065)
( 0.188308606, 0.352213218)
( 0.189854694, 0.359958933)
( 0.191413476, 0.367825219)
( 0.192985056, 0.375813088)
( 0.194569539, 0.383923553)
( 0.196167032, 0.392157626)
( 0.19777764, 0.400516323)
( 0.199401472, 0.40900066)
( 0.201038637, 0.417611655)
( 0.202689243, 0.426350327)
( 0.204353402, 0.435217698)
( 0.206031224, 0.444214791)
( 0.207722821, 0.45334263)
( 0.209428308, 0.462602244)
( 0.211147797, 0.471994661)
( 0.212881403, 0.481520915)
( 0.214629243, 0.491182038)
( 0.216391434, 0.500979067)
( 0.218168093, 0.510913044)
( 0.219959339, 0.520985009)
( 0.221765292, 0.531196008)
( 0.223586072, 0.541547091)
( 0.225421802, 0.552039309)
( 0.227272604, 0.562673716)
( 0.229138601, 0.573451372)
( 0.231019919, 0.58437334)
( 0.232916684, 0.595440685)
( 0.234829022, 0.606654477)
( 0.23675706, 0.61801579)
( 0.238700929, 0.629525703)
( 0.240660758, 0.641185299)
( 0.242636677, 0.652995664)
( 0.24462882, 0.66495789)
( 0.246637319, 0.677073074)
( 0.248662309, 0.689342316)
( 0.250703924, 0.701766724)
( 0.252762302, 0.714347409)
( 0.25483758, 0.727085487)
( 0.256929897, 0.739982082)
( 0.259039393, 0.75303832)
( 0.261166208, 0.766255336)
( 0.263310486, 0.77963427)
( 0.265472368, 0.793176266)
( 0.267652001, 0.806882477)
( 0.26984953, 0.82075406)
( 0.2720651, 0.834792181)
( 0.274298862, 0.848998011)
( 0.276550964, 0.863372727)
( 0.278821556, 0.877917514)
( 0.281110791, 0.892633565)
( 0.283418821, 0.907522079)
( 0.285745801, 0.922584261)
( 0.288091887, 0.937821327)
( 0.290457235, 0.953234497)
( 0.292842003, 0.968825002)
( 0.295246351, 0.984594078)
( 0.29767044, 1.00054297)
( 0.300114432, 1.01667293)
( 0.30257849, 1.03298523)
( 0.305062778, 1.04948113)
( 0.307567464, 1.06616191)
( 0.310092714, 1.08302887)
( 0.312638697, 1.10008329)
( 0.315205584, 1.11732648)
( 0.317793546, 1.13475976)
( 0.320402756, 1.15238446)
( 0.323033389, 1.17020191)
( 0.32568562, 1.18821344)
( 0.328359628, 1.20642043)
( 0.331055589, 1.22482422)
( 0.333773686, 1.2434262)
( 0.3365141, 1.26222774)
( 0.339277013, 1.28123025)
( 0.342062611, 1.30043513)
( 0.34487108, 1.31984379)
( 0.347702607, 1.33945766)
( 0.350557383, 1.35927817)
( 0.353435597, 1.37930679)
( 0.356337442, 1.39954497)
( 0.359263113, 1.41999417)
( 0.362212805, 1.44065589)
( 0.365186714, 1.46153161)
( 0.368185041, 1.48262285)
( 0.371207985, 1.50393113)
( 0.374255749, 1.52545797)
( 0.377328536, 1.54720492)
( 0.380426552, 1.56917353)
( 0.383550004, 1.59136538)
( 0.386699101, 1.61378204)
( 0.389874053, 1.63642511)
( 0.393075072, 1.6592962)
( 0.396302373, 1.68239692)
( 0.399556172, 1.70572892)
( 0.402836686, 1.72929383)
( 0.406144133, 1.75309333)
( 0.409478737, 1.77712908)
( 0.412840719, 1.80140277)
( 0.416230303, 1.82591611)
( 0.419647718, 1.85067082)
( 0.423093191, 1.87566862)
( 0.426566953, 1.90091126)
( 0.430069236, 1.92640051)
( 0.433600274, 1.95213813)
( 0.437160303, 1.97812593)
( 0.440749561, 2.0043657)
( 0.444368288, 2.03085927)
( 0.448016727, 2.05760848)
( 0.451695121, 2.08461517)
( 0.455403716, 2.11188122)
( 0.45914276, 2.13940851)
( 0.462912503, 2.16719894)
( 0.466713197, 2.19525443)
( 0.470545096, 2.2235769)
( 0.474408456, 2.25216832)
( 0.478303537, 2.28103064)
( 0.482230597, 2.31016585)
( 0.4861899, 2.33957595)
( 0.490181711, 2.36926296)
( 0.494206296, 2.39922891)
( 0.498263924, 2.42947586)
( 0.502354867, 2.46000586)
( 0.506479399, 2.49082102)
( 0.510637794, 2.52192344)
( 0.514830331, 2.55331524)
( 0.519057291, 2.58499857)
( 0.523318956, 2.61697558)
( 0.527615611, 2.64924845)
( 0.531947543, 2.68181939)
( 0.536315042, 2.71469061)
( 0.540718399, 2.74786435)
( 0.545157911, 2.78134286)
( 0.549633872, 2.81512841)
( 0.554146582, 2.84922332)
( 0.558696344, 2.88362988)
( 0.563283461, 2.91835043)
( 0.56790824, 2.95338734)
( 0.572570991, 2.98874297)
( 0.577272024, 3.02441972)
( 0.582011655, 3.06042)
( 0.5867902, 3.09674626)
( 0.591607978, 3.13340096)
};
\addplot [red, dash dot]
coordinates {
( 0.01, 1.22268344)
( 0.0100764521, 1.22268347)
( 0.0101534887, 1.22268351)
( 0.0102311143, 1.22268356)
( 0.0103093333, 1.2226836)
( 0.0103881503, 1.22268366)
( 0.0104675699, 1.22268372)
( 0.0105475967, 1.22268378)
( 0.0106282353, 1.22268385)
( 0.0107094904, 1.22268393)
( 0.0107913668, 1.22268402)
( 0.010873869, 1.22268412)
( 0.0109570021, 1.22268423)
( 0.0110407707, 1.22268435)
( 0.0111251797, 1.22268448)
( 0.011210234, 1.22268463)
( 0.0112959386, 1.22268479)
( 0.0113822985, 1.22268496)
( 0.0114693186, 1.22268515)
( 0.0115570039, 1.22268537)
( 0.0116453597, 1.2226856)
( 0.0117343909, 1.22268586)
( 0.0118241028, 1.22268614)
( 0.0119145005, 1.22268644)
( 0.0120055894, 1.22268678)
( 0.0120973747, 1.22268714)
( 0.0121898617, 1.22268755)
( 0.0122830557, 1.22268798)
( 0.0123769623, 1.22268846)
( 0.0124715868, 1.22268898)
( 0.0125669347, 1.22268955)
( 0.0126630116, 1.22269017)
( 0.012759823, 1.22269084)
( 0.0128573745, 1.22269157)
( 0.0129556719, 1.22269236)
( 0.0130547207, 1.22269323)
( 0.0131545268, 1.22269416)
( 0.0132550959, 1.22269517)
( 0.013356434, 1.22269627)
( 0.0134585467, 1.22269746)
( 0.0135614401, 1.22269875)
( 0.0136651202, 1.22270014)
( 0.0137695929, 1.22270165)
( 0.0138748644, 1.22270327)
( 0.0139809407, 1.22270502)
( 0.0140878279, 1.22270691)
( 0.0141955323, 1.22270895)
( 0.0143040602, 1.22271115)
( 0.0144134177, 1.22271351)
( 0.0145236114, 1.22271605)
( 0.0146346474, 1.22271879)
( 0.0147465324, 1.22272173)
( 0.0148592728, 1.22272488)
( 0.014972875, 1.22272827)
( 0.0150873458, 1.2227319)
( 0.0152026918, 1.2227358)
( 0.0153189196, 1.22273997)
( 0.0154360359, 1.22274444)
( 0.0155540477, 1.22274922)
( 0.0156729617, 1.22275433)
( 0.0157927848, 1.2227598)
( 0.015913524, 1.22276563)
( 0.0160351862, 1.22277187)
( 0.0161577786, 1.22277852)
( 0.0162813082, 1.22278562)
( 0.0164057823, 1.22279318)
( 0.0165312079, 1.22280124)
( 0.0166575925, 1.22280982)
( 0.0167849433, 1.22281896)
( 0.0169132678, 1.22282867)
( 0.0170425733, 1.222839)
( 0.0171728674, 1.22284997)
( 0.0173041576, 1.22286163)
( 0.0174364515, 1.222874)
( 0.0175697568, 1.22288712)
( 0.0177040813, 1.22290104)
( 0.0178394328, 1.22291579)
( 0.017975819, 1.22293142)
( 0.018113248, 1.22294797)
( 0.0182517276, 1.22296548)
( 0.0183912659, 1.222984)
( 0.018531871, 1.22300359)
( 0.0186735511, 1.22302428)
( 0.0188163143, 1.22304614)
( 0.018960169, 1.22306922)
( 0.0191051235, 1.22309358)
( 0.0192511862, 1.22311927)
( 0.0193983656, 1.22314636)
( 0.0195466702, 1.2231749)
( 0.0196961086, 1.22320497)
( 0.0198466895, 1.22323663)
( 0.0199984217, 1.22326995)
( 0.0201513138, 1.223305)
( 0.0203053749, 1.22334185)
( 0.0204606137, 1.22338058)
( 0.0206170395, 1.22342127)
( 0.0207746611, 1.22346401)
( 0.0209334878, 1.22350886)
( 0.0210935287, 1.22355592)
( 0.0212547932, 1.22360528)
( 0.0214172906, 1.22365703)
( 0.0215810303, 1.22371126)
( 0.0217460218, 1.22376806)
( 0.0219122747, 1.22382754)
( 0.0220797987, 1.22388979)
( 0.0222486034, 1.22395492)
( 0.0224186987, 1.22402304)
( 0.0225900944, 1.22409425)
( 0.0227628004, 1.22416866)
( 0.0229368269, 1.2242464)
( 0.0231121837, 1.22432757)
( 0.0232888813, 1.2244123)
( 0.0234669297, 1.22450071)
( 0.0236463393, 1.22459292)
( 0.0238271206, 1.22468907)
( 0.024009284, 1.22478927)
( 0.02419284, 1.22489368)
( 0.0243777994, 1.22500242)
( 0.0245641728, 1.22511563)
( 0.0247519711, 1.22523346)
( 0.0249412051, 1.22535605)
( 0.0251318859, 1.22548354)
( 0.0253240245, 1.2256161)
( 0.025517632, 1.22575387)
( 0.0257127197, 1.225897)
( 0.0259092989, 1.22604567)
( 0.0261073809, 1.22620002)
( 0.0263069774, 1.22636023)
( 0.0265080998, 1.22652645)
( 0.0267107598, 1.22669887)
( 0.0269149692, 1.22687766)
( 0.0271207398, 1.22706298)
( 0.0273280836, 1.22725503)
( 0.0275370126, 1.22745397)
( 0.0277475389, 1.22766)
( 0.0279596747, 1.22787329)
( 0.0281734323, 1.22809405)
( 0.0283888241, 1.22832245)
( 0.0286058627, 1.22855869)
( 0.0288245605, 1.22880298)
( 0.0290449304, 1.22905551)
( 0.029266985, 1.22931647)
( 0.0294907373, 1.22958608)
( 0.0297162002, 1.22986454)
( 0.0299433869, 1.23015206)
( 0.0301723104, 1.23044885)
( 0.0304029841, 1.23075512)
( 0.0306354213, 1.23107109)
( 0.0308696356, 1.23139698)
( 0.0311056404, 1.231733)
( 0.0313434496, 1.23207938)
( 0.0315830769, 1.23243634)
( 0.0318245362, 1.23280411)
( 0.0320678415, 1.23318291)
( 0.032313007, 1.23357298)
( 0.0325600467, 1.23397455)
( 0.0328089752, 1.23438785)
( 0.0330598067, 1.23481311)
( 0.0333125559, 1.23525058)
( 0.0335672374, 1.23570048)
( 0.0338238661, 1.23616307)
( 0.0340824567, 1.23663859)
( 0.0343430242, 1.23712727)
( 0.0346055839, 1.23762937)
( 0.0348701509, 1.23814513)
( 0.0351367406, 1.23867479)
( 0.0354053684, 1.23921861)
( 0.0356760499, 1.23977685)
( 0.0359488008, 1.24034974)
( 0.036223637, 1.24093754)
( 0.0365005744, 1.24154051)
( 0.036779629, 1.24215891)
( 0.037060817, 1.24279299)
( 0.0373441548, 1.243443)
( 0.0376296587, 1.24410921)
( 0.0379173454, 1.24479188)
( 0.0382072316, 1.24549126)
( 0.0384993339, 1.24620763)
( 0.0387936694, 1.24694123)
( 0.0390902552, 1.24769234)
( 0.0393891085, 1.24846121)
( 0.0396902466, 1.24924812)
( 0.0399936869, 1.25005332)
( 0.0402994471, 1.25087709)
( 0.0406075449, 1.25171968)
( 0.0409179981, 1.25258137)
( 0.0412308249, 1.25346243)
( 0.0415460432, 1.25436311)
( 0.0418636715, 1.2552837)
( 0.0421837281, 1.25622445)
( 0.0425062316, 1.25718564)
( 0.0428312007, 1.25816753)
( 0.0431586543, 1.2591704)
( 0.0434886113, 1.26019452)
( 0.043821091, 1.26124016)
( 0.0441561125, 1.26230758)
( 0.0444936953, 1.26339706)
( 0.044833859, 1.26450886)
( 0.0451766233, 1.26564327)
( 0.0455220081, 1.26680055)
( 0.0458700335, 1.26798097)
( 0.0462207196, 1.2691848)
( 0.0465740868, 1.27041232)
( 0.0469301555, 1.27166379)
( 0.0472889464, 1.27293949)
( 0.0476504804, 1.27423969)
( 0.0480147784, 1.27556466)
( 0.0483818615, 1.27691467)
( 0.0487517511, 1.27828999)
( 0.0491244685, 1.2796909)
( 0.0495000355, 1.28111767)
( 0.0498784737, 1.28257056)
( 0.0502598052, 1.28404985)
( 0.050644052, 1.28555582)
( 0.0510312365, 1.28708872)
( 0.0514213811, 1.28864884)
( 0.0518145084, 1.29023644)
( 0.0522106412, 1.2918518)
( 0.0526098026, 1.29349518)
( 0.0530120157, 1.29516686)
( 0.0534173037, 1.29686711)
( 0.0538256903, 1.29859619)
( 0.0542371991, 1.30035439)
( 0.0546518539, 1.30214196)
( 0.0550696789, 1.30395918)
( 0.0554906982, 1.30580633)
( 0.0559149363, 1.30768367)
( 0.0563424178, 1.30959146)
( 0.0567731675, 1.31153)
( 0.0572072104, 1.31349953)
( 0.0576445716, 1.31550034)
( 0.0580852765, 1.31753269)
( 0.0585293507, 1.31959685)
( 0.05897682, 1.3216931)
( 0.0594277102, 1.32382171)
( 0.0598820476, 1.32598294)
( 0.0603398585, 1.32817707)
( 0.0608011695, 1.33040437)
( 0.0612660073, 1.33266511)
( 0.0617343988, 1.33495956)
( 0.0622063714, 1.33728799)
( 0.0626819522, 1.33965067)
( 0.063161169, 1.34204788)
( 0.0636440495, 1.34447989)
( 0.0641306217, 1.34694696)
( 0.0646209138, 1.34944938)
( 0.0651149543, 1.35198742)
( 0.0656127719, 1.35456134)
( 0.0661143954, 1.35717142)
( 0.066619854, 1.35981794)
( 0.0671291768, 1.36250117)
( 0.0676423935, 1.36522139)
( 0.0681595339, 1.36797886)
( 0.068680628, 1.37077387)
( 0.0692057059, 1.37360669)
( 0.0697347981, 1.3764776)
( 0.0702679354, 1.37938688)
( 0.0708051486, 1.3823348)
( 0.0713464689, 1.38532164)
( 0.0718919277, 1.38834768)
( 0.0724415567, 1.3914132)
( 0.0729953877, 1.39451849)
( 0.0735534529, 1.39766381)
( 0.0741157846, 1.40084947)
( 0.0746824154, 1.40407572)
( 0.0752533782, 1.40734287)
( 0.0758287062, 1.4106512)
( 0.0764084327, 1.41400098)
( 0.0769925913, 1.41739251)
( 0.0775812159, 1.42082608)
( 0.0781743407, 1.42430196)
( 0.0787720001, 1.42782046)
( 0.0793742286, 1.43138186)
( 0.0799810614, 1.43498645)
( 0.0805925335, 1.43863453)
( 0.0812086804, 1.44232638)
( 0.081829538, 1.44606231)
( 0.0824551421, 1.44984261)
( 0.083085529, 1.45366758)
( 0.0837207355, 1.45753751)
( 0.0843607982, 1.4614527)
( 0.0850057543, 1.46541346)
( 0.0856556412, 1.46942009)
( 0.0863104967, 1.47347289)
( 0.0869703587, 1.47757217)
( 0.0876352655, 1.48171823)
( 0.0883052556, 1.48591138)
( 0.0889803679, 1.49015194)
( 0.0896606416, 1.49444021)
( 0.0903461162, 1.49877651)
( 0.0910368313, 1.50316115)
( 0.0917328271, 1.50759445)
( 0.092434144, 1.51207672)
( 0.0931408225, 1.51660829)
( 0.0938529038, 1.52118948)
( 0.0945704291, 1.52582061)
( 0.09529344, 1.530502)
( 0.0960219785, 1.53523399)
( 0.0967560868, 1.5400169)
( 0.0974958075, 1.54485107)
( 0.0982411835, 1.54973682)
( 0.0989922581, 1.55467449)
( 0.0997490749, 1.55966443)
( 0.100511678, 1.56470696)
( 0.101280111, 1.56980243)
( 0.102054418, 1.57495118)
( 0.102834646, 1.58015356)
( 0.103620839, 1.58540992)
( 0.104413042, 1.59072061)
( 0.105211302, 1.59608597)
( 0.106015664, 1.60150637)
( 0.106826176, 1.60698216)
( 0.107642885, 1.6125137)
( 0.108465838, 1.61810135)
( 0.109295082, 1.62374548)
( 0.110130666, 1.62944646)
( 0.110972638, 1.63520465)
( 0.111821047, 1.64102042)
( 0.112675943, 1.64689416)
( 0.113537374, 1.65282623)
( 0.114405391, 1.65881702)
( 0.115280045, 1.66486691)
( 0.116161385, 1.67097629)
( 0.117049464, 1.67714554)
( 0.117944331, 1.68337505)
( 0.118846041, 1.68966523)
( 0.119754644, 1.69601646)
( 0.120670193, 1.70242914)
( 0.121592742, 1.70890369)
( 0.122522345, 1.71544049)
( 0.123459054, 1.72203997)
( 0.124402924, 1.72870254)
( 0.125354011, 1.7354286)
( 0.126312369, 1.74221858)
( 0.127278054, 1.74907289)
( 0.128251121, 1.75599197)
( 0.129231628, 1.76297623)
( 0.130219631, 1.77002612)
( 0.131215188, 1.77714206)
( 0.132218356, 1.78432448)
( 0.133229193, 1.79157385)
( 0.134247758, 1.79889058)
( 0.135274111, 1.80627514)
( 0.13630831, 1.81372797)
( 0.137350416, 1.82124954)
( 0.138400489, 1.82884028)
( 0.13945859, 1.83650068)
( 0.14052478, 1.84423119)
( 0.141599122, 1.85203228)
( 0.142681677, 1.85990442)
( 0.143772508, 1.8678481)
( 0.14487168, 1.87586378)
( 0.145979254, 1.88395196)
( 0.147095297, 1.89211312)
( 0.148219871, 1.90034775)
( 0.149353043, 1.90865635)
( 0.150494879, 1.91703942)
( 0.151645444, 1.92549746)
( 0.152804806, 1.93403098)
( 0.153973031, 1.94264048)
( 0.155150187, 1.95132649)
( 0.156336343, 1.96008953)
( 0.157531567, 1.96893011)
( 0.158735929, 1.97784876)
( 0.159949499, 1.98684602)
( 0.161172347, 1.99592242)
( 0.162404543, 2.00507851)
( 0.16364616, 2.01431482)
( 0.16489727, 2.02363191)
( 0.166157944, 2.03303033)
( 0.167428257, 2.04251064)
( 0.168708281, 2.0520734)
( 0.169998092, 2.06171918)
( 0.171297763, 2.07144855)
( 0.172607371, 2.08126208)
( 0.173926991, 2.09116036)
( 0.175256699, 2.10114397)
( 0.176596574, 2.11121351)
( 0.177946692, 2.12136956)
( 0.179307132, 2.13161272)
( 0.180677973, 2.14194361)
( 0.182059294, 2.15236283)
( 0.183451176, 2.16287099)
( 0.184853699, 2.17346872)
( 0.186266944, 2.18415663)
( 0.187690994, 2.19493536)
( 0.189125932, 2.20580555)
( 0.190571839, 2.21676782)
( 0.192028801, 2.22782283)
( 0.193496902, 2.23897122)
( 0.194976227, 2.25021366)
( 0.196466861, 2.2615508)
( 0.197968892, 2.2729833)
( 0.199482406, 2.28451184)
( 0.201007491, 2.29613709)
( 0.202544236, 2.30785974)
( 0.204092729, 2.31968047)
( 0.205653061, 2.33159998)
( 0.207225322, 2.34361896)
( 0.208809604, 2.35573812)
( 0.210405997, 2.36795816)
( 0.212014596, 2.38027981)
( 0.213635492, 2.39270378)
( 0.21526878, 2.40523081)
( 0.216914556, 2.41786162)
( 0.218572913, 2.43059695)
( 0.220243949, 2.44343754)
( 0.221927761, 2.45638416)
( 0.223624446, 2.46943755)
( 0.225334102, 2.48259848)
( 0.227056828, 2.49586771)
( 0.228792726, 2.50924602)
( 0.230541895, 2.5227342)
( 0.232304436, 2.53633302)
( 0.234080453, 2.55004329)
( 0.235870047, 2.5638658)
( 0.237673323, 2.57780136)
( 0.239490386, 2.59185078)
( 0.241321341, 2.60601488)
( 0.243166293, 2.6202945)
( 0.245025351, 2.63469045)
( 0.246898622, 2.64920358)
( 0.248786214, 2.66383474)
( 0.250688237, 2.67858478)
( 0.252604802, 2.69345456)
( 0.254536019, 2.70844494)
( 0.256482, 2.72355679)
( 0.258442859, 2.73879101)
( 0.26041871, 2.75414847)
( 0.262409666, 2.76963007)
( 0.264415843, 2.78523672)
( 0.266437358, 2.80096931)
( 0.268474328, 2.81682877)
( 0.270526871, 2.83281601)
( 0.272595106, 2.84893198)
( 0.274679153, 2.8651776)
( 0.276779133, 2.88155383)
( 0.278895168, 2.89806161)
( 0.281027381, 2.91470191)
( 0.283175894, 2.93147569)
( 0.285340834, 2.94838394)
( 0.287522325, 2.96542762)
( 0.289720494, 2.98260774)
( 0.291935468, 2.9999253)
( 0.294167376, 3.01738129)
( 0.296416348, 3.03497674)
( 0.298682514, 3.05271267)
( 0.300966005, 3.07059011)
( 0.303266953, 3.0886101)
( 0.305585493, 3.10677368)
( 0.307921759, 3.12508192)
( 0.310275886, 3.14353588)
( 0.31264801, 3.16213662)
( 0.315038271, 3.18088524)
( 0.317446805, 3.19978281)
( 0.319873753, 3.21883045)
( 0.322319255, 3.23802924)
( 0.324783454, 3.25738032)
( 0.327266492, 3.2768848)
( 0.329768513, 3.29654383)
( 0.332289663, 3.31635853)
( 0.334830088, 3.33633006)
( 0.337389935, 3.35645958)
( 0.339969352, 3.37674826)
( 0.34256849, 3.39719729)
( 0.345187498, 3.41780784)
( 0.347826529, 3.43858111)
( 0.350485737, 3.45951831)
( 0.353165274, 3.48062066)
( 0.355865297, 3.50188939)
( 0.358585963, 3.52332571)
( 0.361327428, 3.54493089)
( 0.364089853, 3.56670618)
( 0.366873396, 3.58865284)
( 0.369678221, 3.61077214)
( 0.372504489, 3.63306537)
( 0.375352365, 3.65553383)
( 0.378222013, 3.67817881)
( 0.3811136, 3.70100164)
( 0.384027294, 3.72400363)
( 0.386963264, 3.74718613)
( 0.38992168, 3.77055048)
( 0.392902713, 3.79409803)
( 0.395906538, 3.81783015)
( 0.398933327, 3.84174823)
( 0.401983256, 3.86585364)
( 0.405056503, 3.89014779)
( 0.408153246, 3.91463209)
( 0.411273663, 3.93930796)
( 0.414417937, 3.96417683)
( 0.41758625, 3.98924014)
( 0.420778785, 4.01449935)
( 0.423995728, 4.03995593)
( 0.427237265, 4.06561135)
( 0.430503584, 4.09146711)
( 0.433794875, 4.11752469)
( 0.437111328, 4.14378562)
( 0.440453137, 4.17025142)
( 0.443820494, 4.19692362)
( 0.447213595, 4.22380378)
};
\addplot [red, dash dot]
coordinates {
( 0.01, 2.81680751e-7)
( 0.0100764521, 3.16313472e-7)
( 0.0101534887, 3.54891923e-7)
( 0.0102311143, 3.97828e-7)
( 0.0103093333, 4.45572377e-7)
( 0.0103881503, 4.98617722e-7)
( 0.0104675699, 5.57502132e-7)
( 0.0105475967, 6.22812813e-7)
( 0.0106282353, 6.95190004e-7)
( 0.0107094904, 7.7533117e-7)
( 0.0107913668, 8.63995463e-7)
( 0.010873869, 9.62008482e-7)
( 0.0109570021, 1.07026733e-6)
( 0.0110407707, 1.189746e-6)
( 0.0111251797, 1.32150106e-6)
( 0.011210234, 1.46667777e-6)
( 0.0112959386, 1.62651643e-6)
( 0.0113822985, 1.80235926e-6)
( 0.0114693186, 1.99565754e-6)
( 0.0115570039, 2.20797923e-6)
( 0.0116453597, 2.44101706e-6)
( 0.0117343909, 2.69659692e-6)
( 0.0118241028, 2.97668687e-6)
( 0.0119145005, 3.28340655e-6)
( 0.0120055894, 3.61903704e-6)
( 0.0120973747, 3.98603135e-6)
( 0.0121898617, 4.3870253e-6)
( 0.0122830557, 4.82484905e-6)
( 0.0123769623, 5.30253915e-6)
( 0.0124715868, 5.82335111e-6)
( 0.0125669347, 6.39077269e-6)
( 0.0126630116, 7.00853763e-6)
( 0.012759823, 7.68064018e-6)
( 0.0128573745, 8.4113501e-6)
( 0.0129556719, 9.20522842e-6)
( 0.0130547207, 1.00671438e-5)
( 0.0131545268, 1.10022898e-5)
( 0.0132550959, 1.20162021e-5)
( 0.013356434, 1.31147777e-5)
( 0.0134585467, 1.43042934e-5)
( 0.0135614401, 1.55914263e-5)
( 0.0136651202, 1.69832739e-5)
( 0.0137695929, 1.84873758e-5)
( 0.0138748644, 2.01117358e-5)
( 0.0139809407, 2.18648446e-5)
( 0.0140878279, 2.37557034e-5)
( 0.0141955323, 2.57938489e-5)
( 0.0143040602, 2.79893774e-5)
( 0.0144134177, 3.03529719e-5)
( 0.0145236114, 3.28959279e-5)
( 0.0146346474, 3.56301814e-5)
( 0.0147465324, 3.85683369e-5)
( 0.0148592728, 4.17236966e-5)
( 0.014972875, 4.51102899e-5)
( 0.0150873458, 4.87429043e-5)
( 0.0152026918, 5.26371163e-5)
( 0.0153189196, 5.68093234e-5)
( 0.0154360359, 6.12767772e-5)
( 0.0155540477, 6.60576165e-5)
( 0.0156729617, 7.11709014e-5)
( 0.0157927848, 7.66366481e-5)
( 0.015913524, 8.24758645e-5)
( 0.0160351862, 8.87105862e-5)
( 0.0161577786, 9.53639129e-5)
( 0.0162813082, 0.000102460046)
( 0.0164057823, 0.000110024327)
( 0.0165312079, 0.000118083274)
( 0.0166575925, 0.000126664623)
( 0.0167849433, 0.000135797365)
( 0.0169132678, 0.000145511788)
( 0.0170425733, 0.000155839514)
( 0.0171728674, 0.000166813544)
( 0.0173041576, 0.000178468295)
( 0.0174364515, 0.000190839642)
( 0.0175697568, 0.000203964962)
( 0.0177040813, 0.000217883173)
( 0.0178394328, 0.000232634775)
( 0.017975819, 0.000248261895)
( 0.018113248, 0.000264808327)
( 0.0182517276, 0.000282319575)
( 0.0183912659, 0.000300842893)
( 0.018531871, 0.000320427329)
( 0.0186735511, 0.000341123767)
( 0.0188163143, 0.000362984967)
( 0.018960169, 0.000386065606)
( 0.0191051235, 0.000410422323)
( 0.0192511862, 0.000436113754)
( 0.0193983656, 0.000463200577)
( 0.0195466702, 0.000491745551)
( 0.0196961086, 0.000521813551)
( 0.0198466895, 0.000553471616)
( 0.0199984217, 0.000586788977)
( 0.0201513138, 0.000621837102)
( 0.0203053749, 0.00065868973)
( 0.0204606137, 0.000697422907)
( 0.0206170395, 0.000738115021)
( 0.0207746611, 0.000780846838)
( 0.0209334878, 0.000825701535)
( 0.0210935287, 0.000872764729)
( 0.0212547932, 0.000922124515)
( 0.0214172906, 0.00097387149)
( 0.0215810303, 0.00102809879)
( 0.0217460218, 0.0010849021)
( 0.0219122747, 0.00114437971)
( 0.0220797987, 0.00120663251)
( 0.0222486034, 0.00127176405)
( 0.0224186987, 0.00133988051)
( 0.0225900944, 0.00141109077)
( 0.0227628004, 0.00148550643)
( 0.0229368269, 0.00156324177)
( 0.0231121837, 0.00164441384)
( 0.0232888813, 0.00172914244)
( 0.0234669297, 0.00181755013)
( 0.0236463393, 0.00190976226)
( 0.0238271206, 0.00200590694)
( 0.024009284, 0.00210611513)
( 0.02419284, 0.00221052056)
( 0.0243777994, 0.00231925978)
( 0.0245641728, 0.00243247217)
( 0.0247519711, 0.00255029992)
( 0.0249412051, 0.00267288803)
( 0.0251318859, 0.00280038435)
( 0.0253240245, 0.00293293951)
( 0.025517632, 0.00307070698)
( 0.0257127197, 0.00321384302)
( 0.0259092989, 0.0033625067)
( 0.0261073809, 0.00351685986)
( 0.0263069774, 0.00367706714)
( 0.0265080998, 0.00384329593)
( 0.0267107598, 0.00401571638)
( 0.0269149692, 0.00419450135)
( 0.0271207398, 0.00437982645)
( 0.0273280836, 0.00457186996)
( 0.0275370126, 0.00477081284)
( 0.0277475389, 0.00497683871)
( 0.0279596747, 0.00519013381)
( 0.0281734323, 0.00541088699)
( 0.0283888241, 0.00563928967)
( 0.0286058627, 0.00587553581)
( 0.0288245605, 0.00611982192)
( 0.0290449304, 0.00637234694)
( 0.029266985, 0.00663331232)
( 0.0294907373, 0.00690292188)
( 0.0297162002, 0.00718138188)
( 0.0299433869, 0.00746890087)
( 0.0301723104, 0.00776568974)
( 0.0304029841, 0.00807196167)
( 0.0306354213, 0.00838793204)
( 0.0308696356, 0.00871381844)
( 0.0311056404, 0.00904984062)
( 0.0313434496, 0.00939622041)
( 0.0315830769, 0.00975318175)
( 0.0318245362, 0.0101209506)
( 0.0320678415, 0.0104997548)
( 0.032313007, 0.0108898243)
( 0.0325600467, 0.0112913908)
( 0.0328089752, 0.0117046879)
( 0.0330598067, 0.0121299509)
( 0.0333125559, 0.0125674171)
( 0.0335672374, 0.0130173253)
( 0.0338238661, 0.0134799159)
( 0.0340824567, 0.0139554311)
( 0.0343430242, 0.0144441145)
( 0.0346055839, 0.0149462113)
( 0.0348701509, 0.0154619682)
( 0.0351367406, 0.0159916332)
( 0.0354053684, 0.0165354557)
( 0.0356760499, 0.0170936865)
( 0.0359488008, 0.0176665777)
( 0.036223637, 0.0182543825)
( 0.0365005744, 0.0188573553)
( 0.036779629, 0.0194757517)
( 0.037060817, 0.0201098284)
( 0.0373441548, 0.020759843)
( 0.0376296587, 0.0214260543)
( 0.0379173454, 0.0221087219)
( 0.0382072316, 0.0228081064)
( 0.0384993339, 0.0235244692)
( 0.0387936694, 0.0242580726)
( 0.0390902552, 0.0250091796)
( 0.0393891085, 0.0257780539)
( 0.0396902466, 0.02656496)
( 0.0399936869, 0.027370163)
( 0.0402994471, 0.0281939287)
( 0.0406075449, 0.0290365234)
( 0.0409179981, 0.0298982139)
( 0.0412308249, 0.0307792677)
( 0.0415460432, 0.0316799525)
( 0.0418636715, 0.0326005367)
( 0.0421837281, 0.0335412889)
( 0.0425062316, 0.0345024782)
( 0.0428312007, 0.0354843739)
( 0.0431586543, 0.0364872459)
( 0.0434886113, 0.037511364)
( 0.043821091, 0.0385569985)
( 0.0441561125, 0.0396244199)
( 0.0444936953, 0.0407138988)
( 0.044833859, 0.0418257061)
( 0.0451766233, 0.0429601128)
( 0.0455220081, 0.0441173901)
( 0.0458700335, 0.045297809)
( 0.0462207196, 0.0465016411)
( 0.0465740868, 0.0477291576)
( 0.0469301555, 0.0489806301)
( 0.0472889464, 0.0502563299)
( 0.0476504804, 0.0515565288)
( 0.0480147784, 0.052881498)
( 0.0483818615, 0.0542315092)
( 0.0487517511, 0.0556068339)
( 0.0491244685, 0.0570077436)
( 0.0495000355, 0.0584345096)
( 0.0498784737, 0.0598874034)
( 0.0502598052, 0.0613666963)
( 0.050644052, 0.0628726596)
( 0.0510312365, 0.0644055645)
( 0.0514213811, 0.0659656822)
( 0.0518145084, 0.0675532838)
( 0.0522106412, 0.0691686404)
( 0.0526098026, 0.0708120228)
( 0.0530120157, 0.0724837019)
( 0.0534173037, 0.0741839487)
( 0.0538256903, 0.0759130338)
( 0.0542371991, 0.077671228)
( 0.0546518539, 0.0794588018)
( 0.0550696789, 0.081276026)
( 0.0554906982, 0.0831231711)
( 0.0559149363, 0.0850005075)
( 0.0563424178, 0.0869083059)
( 0.0567731675, 0.0888468367)
( 0.0572072104, 0.0908163704)
( 0.0576445716, 0.0928171775)
( 0.0580852765, 0.0948495284)
( 0.0585293507, 0.0969136939)
( 0.05897682, 0.0990099444)
( 0.0594277102, 0.101138551)
( 0.0598820476, 0.103299783)
( 0.0603398585, 0.105493913)
( 0.0608011695, 0.107721212)
( 0.0612660073, 0.109981949)
( 0.0617343988, 0.112276398)
( 0.0622063714, 0.114604828)
( 0.0626819522, 0.116967512)
( 0.063161169, 0.119364721)
( 0.0636440495, 0.121796728)
( 0.0641306217, 0.124263804)
( 0.0646209138, 0.126766223)
( 0.0651149543, 0.129304257)
( 0.0656127719, 0.131878179)
( 0.0661143954, 0.134488263)
( 0.066619854, 0.137134782)
( 0.0671291768, 0.139818012)
( 0.0676423935, 0.142538227)
( 0.0681595339, 0.145295701)
( 0.068680628, 0.148090711)
( 0.0692057059, 0.150923533)
( 0.0697347981, 0.153794443)
( 0.0702679354, 0.156703719)
( 0.0708051486, 0.159651639)
( 0.0713464689, 0.16263848)
( 0.0718919277, 0.165664522)
( 0.0724415567, 0.168730045)
( 0.0729953877, 0.171835329)
( 0.0735534529, 0.174980656)
( 0.0741157846, 0.178166307)
( 0.0746824154, 0.181392565)
( 0.0752533782, 0.184659714)
( 0.0758287062, 0.187968038)
( 0.0764084327, 0.191317822)
( 0.0769925913, 0.194709353)
( 0.0775812159, 0.198142918)
( 0.0781743407, 0.201618804)
( 0.0787720001, 0.205137302)
( 0.0793742286, 0.208698701)
( 0.0799810614, 0.212303293)
( 0.0805925335, 0.21595137)
( 0.0812086804, 0.219643226)
( 0.081829538, 0.223379154)
( 0.0824551421, 0.227159453)
( 0.083085529, 0.230984417)
( 0.0837207355, 0.234854347)
( 0.0843607982, 0.238769541)
( 0.0850057543, 0.242730301)
( 0.0856556412, 0.246736929)
( 0.0863104967, 0.25078973)
( 0.0869703587, 0.254889008)
( 0.0876352655, 0.25903507)
( 0.0883052556, 0.263228225)
( 0.0889803679, 0.267468782)
( 0.0896606416, 0.271757053)
( 0.0903461162, 0.276093351)
( 0.0910368313, 0.280477991)
( 0.0917328271, 0.284911289)
( 0.092434144, 0.289393563)
( 0.0931408225, 0.293925133)
( 0.0938529038, 0.298506321)
( 0.0945704291, 0.30313745)
( 0.09529344, 0.307818845)
( 0.0960219785, 0.312550834)
( 0.0967560868, 0.317333745)
( 0.0974958075, 0.322167911)
( 0.0982411835, 0.327053662)
( 0.0989922581, 0.331991336)
( 0.0997490749, 0.336981269)
( 0.100511678, 0.3420238)
( 0.101280111, 0.34711927)
( 0.102054418, 0.352268023)
( 0.102834646, 0.357470405)
( 0.103620839, 0.362726764)
( 0.104413042, 0.368037449)
( 0.105211302, 0.373402814)
( 0.106015664, 0.378823212)
( 0.106826176, 0.384299002)
( 0.107642885, 0.389830543)
( 0.108465838, 0.395418196)
( 0.109295082, 0.401062326)
( 0.110130666, 0.406763301)
( 0.110972638, 0.41252149)
( 0.111821047, 0.418337264)
( 0.112675943, 0.424210998)
( 0.113537374, 0.430143071)
( 0.114405391, 0.436133861)
( 0.115280045, 0.442183752)
( 0.116161385, 0.448293128)
( 0.117049464, 0.454462379)
( 0.117944331, 0.460691894)
( 0.118846041, 0.466982069)
( 0.119754644, 0.473333299)
( 0.120670193, 0.479745985)
( 0.121592742, 0.486220528)
( 0.122522345, 0.492757335)
( 0.123459054, 0.499356814)
( 0.124402924, 0.506019377)
( 0.125354011, 0.512745439)
( 0.126312369, 0.519535417)
( 0.127278054, 0.526389732)
( 0.128251121, 0.533308808)
( 0.129231628, 0.540293073)
( 0.130219631, 0.547342958)
( 0.131215188, 0.554458897)
( 0.132218356, 0.561641326)
( 0.133229193, 0.568890687)
( 0.134247758, 0.576207423)
( 0.135274111, 0.583591982)
( 0.13630831, 0.591044816)
( 0.137350416, 0.598566377)
( 0.138400489, 0.606157124)
( 0.13945859, 0.61381752)
( 0.14052478, 0.621548028)
( 0.141599122, 0.629349118)
( 0.142681677, 0.637221263)
( 0.143772508, 0.645164937)
( 0.14487168, 0.653180622)
( 0.145979254, 0.661268801)
( 0.147095297, 0.669429961)
( 0.148219871, 0.677664594)
( 0.149353043, 0.685973196)
( 0.150494879, 0.694356264)
( 0.151645444, 0.702814303)
( 0.152804806, 0.71134782)
( 0.153973031, 0.719957325)
( 0.155150187, 0.728643334)
( 0.156336343, 0.737406367)
( 0.157531567, 0.746246947)
( 0.158735929, 0.755165601)
( 0.159949499, 0.764162861)
( 0.161172347, 0.773239264)
( 0.162404543, 0.78239535)
( 0.16364616, 0.791631664)
( 0.16489727, 0.800948755)
( 0.166157944, 0.810347176)
( 0.167428257, 0.819827485)
( 0.168708281, 0.829390246)
( 0.169998092, 0.839036024)
( 0.171297763, 0.848765392)
( 0.172607371, 0.858578925)
( 0.173926991, 0.868477205)
( 0.175256699, 0.878460816)
( 0.176596574, 0.888530349)
( 0.177946692, 0.898686399)
( 0.179307132, 0.908929566)
( 0.180677973, 0.919260453)
( 0.182059294, 0.929679671)
( 0.183451176, 0.940187833)
( 0.184853699, 0.950785559)
( 0.186266944, 0.961473473)
( 0.187690994, 0.972252204)
( 0.189125932, 0.983122387)
( 0.190571839, 0.994084661)
( 0.192028801, 1.00513967)
( 0.193496902, 1.01628807)
( 0.194976227, 1.0275305)
( 0.196466861, 1.03886764)
( 0.197968892, 1.05030014)
( 0.199482406, 1.06182868)
( 0.201007491, 1.07345393)
( 0.202544236, 1.08517658)
( 0.204092729, 1.09699731)
( 0.205653061, 1.10891682)
( 0.207225322, 1.1209358)
( 0.208809604, 1.13305496)
( 0.210405997, 1.145275)
( 0.212014596, 1.15759665)
( 0.213635492, 1.17002063)
( 0.21526878, 1.18254765)
( 0.216914556, 1.19517846)
( 0.218572913, 1.20791379)
( 0.220243949, 1.22075439)
( 0.221927761, 1.233701)
( 0.223624446, 1.24675439)
( 0.225334102, 1.25991532)
( 0.227056828, 1.27318455)
( 0.228792726, 1.28656286)
( 0.230541895, 1.30005104)
( 0.232304436, 1.31364986)
( 0.234080453, 1.32736013)
( 0.235870047, 1.34118264)
( 0.237673323, 1.3551182)
( 0.239490386, 1.36916762)
( 0.241321341, 1.38333173)
( 0.243166293, 1.39761134)
( 0.245025351, 1.41200729)
( 0.246898622, 1.42652042)
( 0.248786214, 1.44115158)
( 0.250688237, 1.45590162)
( 0.252604802, 1.4707714)
( 0.254536019, 1.48576178)
( 0.256482, 1.50087363)
( 0.258442859, 1.51610785)
( 0.26041871, 1.53146531)
( 0.262409666, 1.54694691)
( 0.264415843, 1.56255356)
( 0.266437358, 1.57828615)
( 0.268474328, 1.59414561)
( 0.270526871, 1.61013285)
( 0.272595106, 1.62624882)
( 0.274679153, 1.64249444)
( 0.276779133, 1.65887067)
( 0.278895168, 1.67537845)
( 0.281027381, 1.69201875)
( 0.283175894, 1.70879253)
( 0.285340834, 1.72570078)
( 0.287522325, 1.74274446)
( 0.289720494, 1.75992458)
( 0.291935468, 1.77724214)
( 0.294167376, 1.79469813)
( 0.296416348, 1.81229358)
( 0.298682514, 1.83002951)
( 0.300966005, 1.84790695)
( 0.303266953, 1.86592694)
( 0.305585493, 1.88409053)
( 0.307921759, 1.90239876)
( 0.310275886, 1.92085272)
( 0.31264801, 1.93945346)
( 0.315038271, 1.95820208)
( 0.317446805, 1.97709965)
( 0.319873753, 1.99614729)
( 0.322319255, 2.01534608)
( 0.324783454, 2.03469716)
( 0.327266492, 2.05420165)
( 0.329768513, 2.07386067)
( 0.332289663, 2.09367537)
( 0.334830088, 2.1136469)
( 0.337389935, 2.13377642)
( 0.339969352, 2.15406511)
( 0.34256849, 2.17451413)
( 0.345187498, 2.19512468)
( 0.347826529, 2.21589795)
( 0.350485737, 2.23683516)
( 0.353165274, 2.25793751)
( 0.355865297, 2.27920623)
( 0.358585963, 2.30064256)
( 0.361327428, 2.32224774)
( 0.364089853, 2.34402302)
( 0.366873396, 2.36596968)
( 0.369678221, 2.38808898)
( 0.372504489, 2.41038221)
( 0.375352365, 2.43285067)
( 0.378222013, 2.45549565)
( 0.3811136, 2.47831848)
( 0.384027294, 2.50132047)
( 0.386963264, 2.52450297)
( 0.38992168, 2.54786732)
( 0.392902713, 2.57141487)
( 0.395906538, 2.59514699)
( 0.398933327, 2.61906507)
( 0.401983256, 2.64317048)
( 0.405056503, 2.66746463)
( 0.408153246, 2.69194893)
( 0.411273663, 2.7166248)
( 0.414417937, 2.74149367)
( 0.41758625, 2.76655698)
( 0.420778785, 2.79181619)
( 0.423995728, 2.81727277)
( 0.427237265, 2.84292819)
( 0.430503584, 2.86878395)
( 0.433794875, 2.89484153)
( 0.437111328, 2.92110246)
( 0.440453137, 2.94756826)
( 0.443820494, 2.97424047)
( 0.447213595, 3.00112062)
};
\end{loglogaxis}

